PrefillOnly: An Inference Engine for Prefill-only Workloads in Large Language Model Applications

Besides typical generative applications, like ChatGPT, GitHub Copilot, and Cursor, we observe an emerging trend that LLMs are increasingly used in traditional discriminative tasks, such as recommendation, credit verification, and data labeling. The key characteristic of these emerging use cases is that the LLM generates only a single output token, rather than an arbitrarily long sequence of tokens. We call this prefill-only workload. However, since existing LLM engines assume arbitrary output lengths, they fail to leverage the unique properties of prefill-only workloads. In this paper, we present PrefillOnly, the first LLM inference engine that improves the inference throughput and latency by fully embracing the properties of prefill-only workloads. First, since it generates only one token, PrefillOnly only needs to store the KV cache of only the last computed layer, rather than of all layers. This drastically reduces the GPU memory footprint of LLM inference and allows handling long inputs without using solutions that reduces throughput, such as cross-GPU KV cache parallelization. Second, because the output length is fixed, rather than arbitrary, PrefillOnly can precisely determine the job completion time (JCT) of each prefill-only request before it starts. This enables efficient JCT-aware scheduling policies such as shortest remaining job first. PrefillOnly can process upto 4x larger queries per second without inflating average and P99 latency.

==> tex-files/abstract-junchen.tex <==
Besides typical generative applications, like ChatGPT, Github Copilot, and Cursor, we observe an emerging trend that LLMs are increasingly used in traditional discriminative tasks, such as recommendation, credit verification, and data labeling. 
The key characteristic of these emerging use cases is that the LLM generates only a {\em single} output token, rather than an arbitrarily long sequence of tokens. We call this {\em prefill-only} workloads.
However, existing LLM inference engines assume arbitrary output lengths, rather than prefill-only workloads. 
In this paper, we present \name, the first LLM inference engine that drastically improves the throughput and delay by fully embracing the prefill-only characteristics. 
First, to generate only one token, \name only needs to store the KV cache of only the last computed layer, rather than of all layers. This significantly reduces the GPU memory usage and avoids cross-GPU tensor parallelization. 
Second, because the output length is fixed, rather than arbitrary, \name could precisely determine the job completion time of each prefill-only request before it starts. 
This enables optimal scheduling policies such as shortest remaining job first. 
\name can process upto $4\times$ larger query per second without inflating average and P99 latency, while handling requests up to $7\times$ longer without latency inflation.

==> tex-files/characterizaton.tex <==
%!TEX root = ../paper.tex
%!TEX spellcheck = en_US


\tightsection{Motivation}
\label{sec:characterization}

% \begin{outline}

% Motivation

% \1 Satellite imagery applications are important.
% \1 However, the downlink capacity is not sufficient to download all images captured by the satellite.
% \1 To handle limited downlink capacity, there are two types of satellite systems exist.
%     \2 Mission-based satellite system: people download imagery from the satellite after specifying a specific application. 
%         \3 Benefit: allow the satellite to run application-specific filtering, which can filter out a lot of imagery. 
%         \3 Drawback: cannot query historical data (unless someone has queried the same data before).
%     \2 General-purpose satellite system: to support the query of historical data, some systems instead download the data to the ground without specifying concrete applications. However, to extend limited downlink capacity, they have to build highly powerful satellites (e.g. Sentinel-2), send more satellites or build more ground stations. All of these choices are extremely expensive. 
% \1 We aim to compress the satellite imagery on general-purpose satellite so that more images can be downloaded from existing general-purpose satellite system (which allows more frequent ground data downloading), or reduce the cost of expanding the downlink capacity for future general-purpose satellite system.
% \jc{i like the problem statement, but the objective (measure of success) can be made more direct. instead of saying downloading more images or reducing cost, how about we say "increasing the image freshness and quality at each location given a given set of base stations currently deployed" or "reducing the number of base stations while achieving the same image freshness and quality at each location"}
% \1 Problem formulation: maximize the PSNR of observed ground data, subject to the limited resource constraint of general purpose satellite:
%     \2 Limited downlink: total downlink capacity is about ?? MB during each contact to the ground.
%     \2 Limited storage: storage is only 720 GB.
%     \2 Limited compute: computation power is only ?TFLOPs per image.
%     \2 Limited uplink
%     \2 \kt{All the data above need to be filled and cited. Let me search the spec of planetscope satellites and.}
% \jc{to highlight the potential of a better solution, it would help to contrast two numbers: 
% (1) how often is an image captured in each location by {\em any} satellite, and 
% (2) how often is the image in each location refreshed now. 
% supposably the former is much higher than the latter?}
% \1 Research opportunity: a lot of geographical contents remain unchanged between two consecutive satellite visit. This inspires change-based encoding. Several prior works in this direction.
% \1 Key design question: how to obtain reference images on-board.
% Prior work assumes that reference images of all locations are available on the satellite. 
% However, the reference images need to be compressed for >200x to store all these reference images on-board, which makes change-based encoding almost useless.
% % \1 We calculate that, to fit into the on-board storage capacity, the reference images need to be compressed by more than 200x compression.
% \1 To quantify the effect of 200x-compressed reference image, we perform a measurement experiment.
%     \2 Data: image pairs from Sentinel-2 dataset with time delta < 10 days. 
%     \2 X-axis: compression ratio of reference image
%     \2 Y-axis: \% of areas need to be downloaded in order to cover 99\% change (change: pixel diff > 0.002 compared to reference image, all pixel values normalized to [0,1]).
%     \2 Takeaway: when the reference images are compressed by >200x, more than half of the geographical areas need to be downloaded  even when the actual change is only 5\%.
% % \1 We advocate for a new design: the satellite only keep the reference images for a small subset of locations, the ground timely update the reference images on the satellite via uplink.

% % \1 Satellite imagery is important
% %     \2 Note: we focus on applications that observe the ground rather than the atmosphere.
% % \1 However, the downlink capacity is not sufficient to download all images captured by the satellite.
% % \1 To handle limited downlink capacity, there are two types of satellite systems exist.
% %     \2 Mission-based satellite system: people download imagery from the satellite after specifying a specific application. 
% %         \3 Benefit: allow the satellite to run application-specific filtering, which can filter out a lot of imagery. 
% %         \3 Cons: 
% %     \2 Cannot download all images: downlink capacity is ??x smaller than daily generated image \kt{I remember Kodan has some information for this}
% %     \2 Storage space is limited: can only keep ?? hours of observed imagery on-board.
% %     \2 Compute power is limited: only ?? CPU available
% % \1 Problem formulation: maximize the PSNR of observed ground data, subject to the limited downlink bandwidth, storage and compute power of satellite.
% %     \2 Why PSNR: let me check if prior work has a justification for this
% % \1 Two types of prior work exists to handle the downlink bottleneck:
% %     \2 Application-specific filtering (Kodan, OEC) ==> Will filter out data that are potentially useful for other applications (examples). 
% %     \2 Change-based encoding (SatRoI, VirtualBackground): Not directly applicable on the satellite.
% %         \kt{Conventional belief: uplink for controls, too limited for reference images.}
% %         \kt{Eval: are we fitting into the eval budget}
% %         \3 These approach requires accessing reference images for all geographical locations on the satellite to detect changes.
% %         \3 To fit into limited on-board storage, these images need to be compressed for >500x (a placeholder number), which requires downsampling the reference image 128x, width and height, which significantly degrades the change detection quality.
% %         \3 An experiment to support this argument
% %             \4 X-axis: \% of areas need to be downloaded
% %             \4 Y-axis: \% of changes (defined as pixels w/ pixel difference > 100) covered 
% %             \4 Curves: change detection w/ different compression ratio of reference image
% %             \4 Takeaway: to download 95\% of the changes, it need to download ??\% geographical areas, ?x more than the areas actually need to be downloaded.
% \end{outline}


We start with the background on satellite imagery and earth observation satellite constellations.



\tightsubsection{Background}
% \subsection{Background on earth observation satellite constellations}
\label{subsec:satellite-connectivity}
% \kt{More text here talking about LEO satellite constellations}



\begin{figure}
    \centering
    \includegraphics[width=0.48\columnwidth]{figures/earth-orbit-illustration.pdf}
    \tightcaption{Illustration of a LEO satellite constellation: the satellites follow a sun-synchronous orbit, and the ground station downloads imagery data from a satellite when the satellite passes through it.
    % , where the constellation puts its satellites on a sun-synchronous orbit and potentially downloads data to the ground when any of the satellites pass through the area with ground station connectivity.
    }
    \label{fig:leo-orbit-illustration}
\end{figure}


% \kt{Peder/Shadi: I wrote a version of text here to cover more backgrounds on LEO satellite constellations. Feel free to edit this part if there are factual errors, or there are things we should/should not cover.}
Many applications can benefit from frequently updated (\eg daily) and high-resolution satellite imagery.
For example, precision agriculture ideally needs daily access to satellite imagery with each pixel corresponding to a $5\mathrm{m}\times5\mathrm{m}$ area on Earth~\cite{agriculture-daily,agriculture-daily2} to help timely decisions on the distribution of fertilizers, pesticides, and water. 
Also, wildfire monitoring requires the imagery to be updated frequently with sufficient resolution to promptly detect and respond to fire outbreaks, mitigating potential damage~\cite{serval}.


To provide fresh, high-resolution satellite imagery, many LEO satellites (\eg >100 satellites~\cite{planet}) are deployed to form satellite constellations. 
% \edit{This gives more background information to LEO constellation that can address reviewer A's concern on time-of-the-day difference, reviewer C's concern on why satellite are not able to always communicate to the ground, and reviewer D's concern on satellite orbit}{
Figure~\ref{fig:leo-orbit-illustration} shows an illustrative example of a LEO satellite constellation, where multiple satellites are located in a sun-synchronous orbit\footnote{A sun-synchronous orbit ensures that each location on Earth is  revisited once per day, at approximately the same time local time, allowing the constellation to capture images with similar illumination condition once per day.} and these satellites can potentially stream data to the ground when they are close enough to one of the ground stations (we only plot one ground station in the figure for simplicity).
% }

We characterize two features of such LEO satellite constellations:
% three-fold:\jc{i'd tune it down a bit. maybe just explain the features of LEO and explain why they are {\em could} be good for high res high coverage (instead of contrasting them with other satellite types).}
\begin{packeditemize}
    \item \textit{High-resolution imagery}: LEO satellites are close to the ground (due to their low earth orbits) and can capture imagery with low ground-sampling distance (GSD for short, lower GSD means higher resolution).
    % \jc{not sure if we want to compare with medium or high earth orbit ones. it seems to invite the question why can't they just get higher resolution cameras, which is not the point anyway}
    \item \textit{Frequent revisit}:
    With a large number of satellites, any location on the earth's surface will be frequently revisited (\eg daily ~\cite{planet}), while a single satellite can only revisit one location once every ten days~\cite{sentinel-2-revisit}.
    % of one location being captured is significantly improved.
    % Concretely, a single satellite captures imagery for one location once every 10 days~\cite{sentinel-2-revisit}, while DOVEs constellation~\cite{planet} revisits any location on Earth daily (since it\jc{this sounds like the constellation only has one satellite?} orbits on syn-synchronous orbit, which strike through every location on the Earth daily).
    % \item \textit{More downlink capacity}:
    % By increasing the number of satellites, the total downlink capacity of the whole constellation (which is the sum of each individual satellite's downlink capacity) will increase, allowing more imagery to be downloaded to the ground.
    % \yh{The title "\textit{More downlink capacity}" is a bit contradicting to section 2.2 (i.e., the downlink is the bottleneck). The title makes me feel like "there is much more downlink capacity than before", but I guess that's not what we want to say here}
    % While each single satellite can only contact one ground station (\ie there may be cases that the next satellite connects the same ground station hours after the previous satellite finishes its connection), large-scale LEO constellations can saturate the ground station, thus allowing more imagery to be downloaded to the ground.
    % \kt{Saturate is an awkward word but I don't have a better way to show why downlink is improved?}
    % increasing the number of satellites, the  has longer ground contact time in total, allowing downloading more imagery to the ground.
    % This longer contact time is because other satellites in the same constellation can start connecting the ground station one-by-one.
\end{packeditemize}
% While deploying, these satellites typically orbit the Earth on a sun-synchronous orbit (as illustrated in Figure~\ref{fig:leo-orbit-illustration}). 
% This orbit will strike through every location on the Earth daily, at approximately the same time as that location.
% Thus, with a sufficient amount of satellites in this orbit, one can capture every location on the Earth daily~\cite{planet}.





% where multiple satellites are located in a sun-synchronous orbit\footnote{A sun-synchronous orbit ensures that each location on the earth is approximately revisited once per day, at approximately the same time local time, allowing the constellation to capture images with similar illumination condition once per day.} and these satellites can potentially stream data to the ground when they are close enough to one of the ground stations (we only plot one ground station in the figure for simplicity).

Note that in the following text, we denote \textit{the ground} as the ground stations that the constellation can potentially contact and the computation and networking infrastructures around these ground stations.

% \jc{let's just briefly mention the large body of database research on satellite-image management, and clarify that this paper focuses on a different challenge. also, that body of work should be mentioned (again briefly) in the related work section}
% \kt{Mention DB work on satellite imagery management}



% First, 
% Second, large-scale LEO constellation can significantly increase the total ground contact time for the whole constellation, allowing downloading more imagery data to the ground station~\cite{kodan,serval}.


% With a sufficient amount of satellites, this sun-synchronous orbit allows capturing images for any location on Earth daily, at approximately the same time.
% This is because the satellites typically orbit the Earth on Sun-synchronous Orbit, 
% large-scale constellation provides continuous high-resolution imagery, we take DOVE constellations~\cite{planet} from Planet as an example.
% DOVEs constellation provides imagery at a ground sampling distance (the distance between the center of nearby pixels, GSD for short) of 10 meters.
% This constellation orbits the earth using a Sun-synchronous Orbit, which can cover all locations on Earth while making sure a location is revisited daily, at approximately the same local time of that location.



% Satellite imagery plays a crucial role in a wide range of applications such as precision agriculture~\cite{mulla2013twenty, hank2019spaceborne,planet-digital-agriculture,digital-agriculture1}, environmental monitoring~\cite{manfreda2018use, tucker2000strategies, tralli2005satellite, cunjian2001extracting,environment-monitoring1}, and automatic road detection~\cite{kopsiaftis2015vehicle, van2018spacenet,automatic-road-detection}.

% To effectively respond to the latest changes happening on the ground, these applications require access to high-resolution satellite imagery that is frequently updated. 
% We note that in satellite imagery, image resolution is typically measured by ground sampling distance between neighboring pixels (GSD for short) lower GSD means higher resolution.

% For example, precision agriculture demands daily access to satellite images with a GSD of 1 - 5 meters or lower~\cite{agriculture-daily,agriculture-daily2}, enabling timely decisions concerning the distribution of fertilizers, pesticides, and water. 
% Similarly, wildfire monitoring requires the imagery to be updated every few minutes with sufficient resolution to promptly detect and respond to fire outbreaks, mitigating potential damage.

% To quickly react to the latest changes on the ground, many applications need access to \textit{high-resolution} imagery data updated at \textit{high frequency}.
% Typically, the resolution of an image is measured by ground sampling distance (defined as the distance between the center of nearby pixels, GSD for short). 


% To make the requirements of freshness and resolution more concrete,
% precision agriculture needs daily access~\cite{agriculture-daily,agriculture-daily2} to high-resolution satellite imagery, with a GSD of 1 - 5 meters or lower~\cite{application-GSD}) to timely determine which areas need more fertilizers, pesticides, and water.
% Similarly, wild fire monitoring applications ideally need the satellite imagery to be updated once every few minutes, with enough resolution to timely identify the start of wild fire, in order to contain the damage. %the risk for human lives.


% \jc{a bit too hand-way right now. need more concrete and stronger motivation, e.g., how would higher fidelity/coverage/freshness images improve those applications if they are available?}

% \jc{also it's a good place to clarify the diff w.r.t LEO satellites for communication. this could be in 2.2 too}
% However, limited by the downlink capacity, the satellite imagery captured by the satellite cannot be fully downloaded by the satellite.

% Further, having frequent access to the ground is crucial to these applications, 


% \subsection{LEO satellite constellation}
% \jc{kuntai, like we discussed, we probably don't need a separate subsection anymore. we can just explain the specs of current satellites (including mission-specific and general-purpose, and why general purpose is as popular and as important}
% \kt{This section aims to set up the stage for general LEO satellite constellations, }

% To provide high-resolution satellite imagery with high frequency, people deploy low earth orbit satellites (LEO satellites for short) and set up large-scale satellite constellations for earth observation purposes.
% % For example, Planet's DOVEs constellation contains about 130 satellites that provide high-resolution satellite imagery (with a GSD of 3m) every day.

% We want to point out four characteristics of recent LEO satellite constellations:
% \begin{packeditemize}
%     \item \textbf{\textit{Large constellation size}}: Recent LEO satellite constellations (\eg DOVEs constellation~\cite{planet} and Lemur-2 constellation~\cite{lemur2}) contain more than 100 satellites.
%     \item \textbf{\textit{High-resolution imagery}}: These satellite constellations provide much higher resolution imagery (\eg 3-meter GSD in DOVEs constellation~\cite{dove-constellation}), where traditional satellites typically has much lower resolution (\eg 250-meter GSD in MODIS~\cite{MODIS}).
%     \item \textbf{\textit{High ground access frequency}}: Due to the large constellation size, these constellation can photo the earth frequently (\eg daily in DOVEs constellation~\cite{planet}).
%     \item \textbf{\textit{Downlink-heavy connectivity}}: LEO satellites have high downlink capacity (\eg 200 Mbps for DOVEs constellation at year 2017~\cite{dove-uplink-downlink}) but limited uplink capacity (\eg 250 kbps in DOVEs constellation~\cite{dove-uplink-downlink}).
%     Moreover, earth-observation LEO satellites typically do \textbf{\textit{not}} have inter-satellite connections.
% \end{packeditemize}



% More recently, within the last 5-10 years, the emergence of large LEO constellations, comprising of hundreds of satellites, has been driven by lower launch and manufacturing costs of small satellites. For example, Planet’s Dove constel- lation for Earth imagery is composed of nearly 200 low-cost cubesats ('shoebox-sized’ satellites) with off-the-shelf com- ponents. Our work focuses on these modern constellations for Earth observation. These modern constellations differ from traditional satellite constellations in three ways:
% • Constellation Size: Modern satellite constellations (e.g., Planet Inc. [25], Spire Inc. [2], etc.), consist of hundreds of satellites as opposed to few satellites in traditional constellations. This allows modern constellations to get more frequent imagery of any part of Earth with revisit frequency of few hours as opposed to a delay of several days from traditional constellations.



\tightsubsection{Downlink bottleneck and our objective}


% \jc{again, a little bit more details are needed. what type of connection is it? how long each connection is? does bandwidth vary over time? do we take them into account or not? how many bands? how are satellite images different from normal RGB images? }

% \jc{this is also a good place to explain how often a satellite visits the ground station? how often does it photograph a region?}

% Network Pipeline: Finally, we provide a brief description of satellite network pipeline as context for the rest of the paper. LEO satellites for Earth observation operate in polar orbits and go around the Earth once every 1.5 hours appoximately. During each orbit, they pass over a different part of the Earth due to Earth’s rotation. The data from these satellites is usu- ally downloaded using few dedicated ground stations with Gbps link capacities [24]. Due to a satellite’s orbital motion, it can contact each ground station four to six times a day, with each contact lasting up to ten minutes. To improve down- load latency and increase the number of contacts, recent work has proposed distributed ground station designs with multiple general-purpose ground stations [56,57]. In the industry, Ama- zon and Microsoft have launched ground-station-as-a-service platforms [6, 43], wherein satellite operators can rent time on existing ground stations to download data from satellites.


% \mypara{Characterizing downlink}
% We first characterize the downlink of earth observation satellites, using technical specifications of DOVEs constellation~\cite{planet} in the year 2017.
% During each ground contact, the downlink bandwidth is around 200 Mbps~\cite{dove-uplink-downlink} during sunny days, and the ground contact time is around 10 minutes~\cite{leoconn,ground-contact-time,satellite-ground-contact-time}.
% As a result, during each ground contact time, 



% A recent study~\cite{kodan} has shown that only 2\% of the total images observed by the satellite can be downloaded to the ground under the current downlink capacity, illustrating that the downlink capacity is 50$\times$ smaller than the amount of data observed by the satellite.
% As a result, even though each location will be photoed once per less than 1 hour in average, the ground can only obtain the images daily~\cite{planet}.


% \kt{Is there any data related to the number of ground contacts in planet...}


% We first characterize the downlink from the satellite to the ground. 

% \kt{Peder/Shadi, is there any other numbers we can quote here to support that downlink is limited?}

\mypara{Downlink capacity gap}
Despite more images being captured by the satellites, only a small fraction of data are downloaded to the ground due to 
% existing earth observation LEO constellations are bottlenecked by the 
the limited capacity of the downlink (satellite-to-ground)~\cite{kodan,serval,falcon}.
% \footnote{To put this gap in perspective, we use the data from the Doves constellation in 2017~\cite{planet}, where each satellite image covers an area of 400~km$^2$(assuming 6600×4400 resolution~\cite{planet-ground-sampling-distance} and a GSD of 3.7 meters~\cite{planet-ground-sampling-distance}) so after scanning the whole earth's surface, we would accumulate 1.275 million images or 191.25 TB of data (with each image being 150~MB~\cite{planet-image-size}).
% To estimate how much data can be downloaded, we make the idealized assumption that the satellite always has a stable connection of 200~Mbps~\cite{dove-uplink-downlink} with a ground station. 
% Now, each satellite scans the whole Earth's surface every ten days~\cite{sentinel-2-revisit}, so under the idealized assumption, the satellite can only transmit 21.6~TB of data to the ground, which is less than 12\% of the 191.25~TB of data accumulated during that period of time.}
Specifically, we refer to {\em downlink bandwidth} as the average download speed from satellites to the ground during each ground contact.
The exact gap between the downlink capacity and the imagery data varies with the constellation, and a recent study shows only about 2\% of the images captured by satellites are actually downloaded to the ground~\cite{kodan}.
% \yh{The example is clear but a bit wordy here. Maybe we can use a table or a figure to illustrate the numbers?}




\begin{comment}
we can estimate this gap using the 2017 data from the DOVEs constellation~\cite{planet}.
% this downlink bottleneck by analyzing the downlink supply and demand.
% \mypara{}
The Earth's surface is about 510 million square kilometers.
% ~\cite{earth-surface}. 
Assuming that each satellite image is 150~MB~\cite{planet-image-size} and covers an area of 400 square kilometers\footnote{This estimate is based on a resolution of 6600×4400 pixels~\cite{planet-ground-sampling-distance} and a GSD of 3.7 meters~\cite{planet-ground-sampling-distance}.}, then covering the Earth's surface takes 1.275 million images or 191.25 TB of data in total. 
% has a resolution of 6600×4400 pixels~\cite{planet-ground-sampling-distance} and a GSD of 3.7 meters~\cite{planet-ground-sampling-distance}, each image can covering approximately 400 square kilometers.
% This translates to about 1.275 million images to cover the entire Earth, amounting to a total of 191.25 TB (since each image is approximately 150 MB~\cite{planet-image-size}).
Now, let us make an {\em idealized} assumption that the satellite is \textit{always} connecting with a ground station, 
% the weather is {\em always} clear between the satellite and the ground station, 
so the satellite can enjoy a bandwidth of 200 Mbps~\cite{dove-uplink-downlink} 24/7. 
Since each satellite scans Earth's surface every ten days~\cite{sentinel-2-revisit}, that means it can at most transmit 21.6~TB of data down to the ground.
Thus, even under such an idealized downlink connectivity, the downlink capacity is 10$\times$ lower than the demand to download all imagery data. 
\end{comment}

% the average downlink bandwidth during a clear day (no cloud blocking) is around 200 Mbps~\cite{dove-uplink-downlink}. 

% satellite's earth orbit cycle of 10 days~\cite{sentinel-2-revisit}, 
% Thus, it can transmit around 21.6 terabytes (TB) of data to Earth in this period.
% \mypara{Downlink demand}

% Consequently, the available downlink supply is approximately 9 times smaller than the demand, even assuming constant satellite-ground contact. Previous studies also shows a similar phenomenon that only about 2\% of the images captured by satellites are actually downloaded to the ground~\cite{kodan}.



Further, the downlink demand is constantly growing, with higher resolution (\eg a GSD of 0.5m~\cite{high-resolution-satellite-imagery}) and more bands found to be useful (\eg vegetarian red edge band and water vapor band~\cite{sentinel-2-bands}).
In contrast, the downlink grows slowly due to the long deployment cycle of satellites.
These trends suggest that the gap between the demand for downlink bandwidth and its actual capacity will likely persist if not increase.

% \kt{Say sensor and resolution is going higher and higher}


% However, most of the observed satellite imagery data are \textbf{\textit{not}} received by the ground due to limited downlink (\ie satellite-to-ground link) capacity. We provide a ballpark analysis here.


% \mypara{Downlink supply}
% We take the statistics from DOVEs constellation in the year 2017 as an example to characterize the downlink.
% During each ground contact, the downlink bandwidth is around 200 Mbps~\cite{dove-uplink-downlink} during sunny days.
% As the satellite typically iterates over the full earth once every 10 days~\cite{sentinel-2-revisit}, the satellite can download 21.6 TB worth of data during 10 days.

% \mypara{Downlink demand}
% The total area of the earth's surface is about 510 million km$^2$~\cite{earth-surface}. Each image captured by the satellite is of resolution 6600$\times$4400~\cite{planet-ground-sampling-distance}, with a ground sampling distance of 3.7 meter~\cite{planet-ground-sampling-distance} and a file size of 150 MB~\cite{planet-image-size}.
% As a result, each image covers about 400 km$^2$ areas, thus the earth's surface corresponds to 1.275 million images, totaling 191.25 TB.

% As a result, the downlink supply is $9\times$ smaller than the downlink demand even if the satellite is always in contact with the ground.
% Prior work also observes similar phenomena, that only 2\% of the images observed by the satellite is actually downloaded to the ground~\cite{kodan}.






% \mypara{Downlink bottleneck}
% However, this amount of downlink bandwidth is far less enough to download all observed imagery on the satellite: 
% Earth-observation LEO satellites go around the Earth once every 90 minutes~\cite{orbital-time} but their orbit changes during each round.
% As a result, it can typically contact each ground station 4-6 time




% However, the reality is that most satellite imagery data are not received on the ground due to {\em limited downlink capacity}.




% \mypara{Uplink}
% The satellite also has uplink connectivity.
% Different from downlink that is used to stream satellite imagery data, current uplink is mainly used to stream the control messages, and thus has very limited bandwidth.
% Concretely, for one Planet satellite, the uplink is only 250 kbps, 800$\times$ smaller than its downlink.



% \mypara{Inter-satellite link}
% \kt{Finish here.}
% We point out that current earth 




% To handle such downlink bottleneck, different satellite constellations adopt different approaches. We classify them into two categories.
% There are two types of existing systems for satellite imagery, which handles the downlink bottleneck in different manner.


% However, satellites are now generating much more data than the amount of data that ground station can download.

% For example, a Sentinel-2 satellite generates 1.6 TB~\cite{sentinel-data-generation-rate} data per day.
% But the downlink capacity is only 0.3 TB per day on average\footnote{The connection between the satellite and the ground happens 6-8 times per day, and each time the contact lasts between 5 to 15 minutes~\cite{satellite-ground-contact-time}. The downlink bandwidth of such a connection is 560Mbps~\cite{sentinel-data-generation-rate}, resulting in a daily downlink capacity of 0.3TB on average}, 5x smaller than the daily generated data.
% \kt{I use Sentinel-2 satellite as the example, but Sentinel-2 satellites are too expensive to sufficiently highlight the gap between generated data and downlink capacity. We should use other satellites (like DOVEs constellation from planetscope) as the example.}
% The gap between the daily generated data and daily downlink capacity will be even larger if the ground-satellite connection is partially blocked by the cloud.



%\subsection{Optimization objective}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
% Section                                                                                & Properties                 & Values                                                  \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Connectivity\end{tabular}} & Ground contact duration    & \textit{10 minutes}~\cite{leoconn,ground-contact-time}  \\ \cline{2-3} 
%                                                                                        & Ground contact per day     & \textit{7 times}~\cite{ground-contact-time}             \\ \cline{2-3} 
%                                                                                        & Uplink bandwidth           & 250 kbps~\cite{dove-uplink-downlink}                    \\ \cline{2-3} 
%                                                                                        & Downlink bandwidth         & 200 Mbps~\cite{dove-uplink-downlink}                    \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Hardware\end{tabular}}     & On-board storage           & \textit{30 GB minimum}\footnotemark{}                   \\ \cline{2-3} 
%                                                                                        & On-board CPU               & \textit{EDGE 1U processor}~\cite{satellite-edge-cpu}    \\ \cline{2-3} 
%                                                                                        & Computation time per image & \textit{22 seconds}~\cite{kodan}                        \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Image\end{tabular}}        & Image resolution           & 6600$\times$4400~\cite{planet-ground-sampling-distance} \\ \cline{2-3} 
%                                                                                        & Image channels             & RGB + InfraRed~\cite{planet-ground-sampling-distance}   \\ \cline{2-3} 
%                                                                                        & Image file size            & \textit{150 MB}~\cite{planet-image-size}               \\ \cline{2-3} 
%                                                                                        & Ground sampling distance   & 3.7 meters~\cite{planet-ground-sampling-distance}       \\ \hline
% \end{tabular}
% \caption{Characterizing the specifications of DOVEs constellation from year 2017 to year 2018. Some of the data are not publically available and we infer them from other sources (we \textit{italicized} the data that we inferred).}
% \label{tab:hardware-specs}
% \end{table}




% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|}
% \hline
% Properties      & Values                         \\ \hline
% Ground contact duration      & \textit{10 minuites}~\cite{leoconn,ground-contact-time}                        \\ \hline
% Ground contact per day         & \textit{7 times}~\cite{ground-contact-time}                           \\ \hline
% Uplink bandwidth         & 250 kbps~\cite{dove-uplink-downlink}                           \\ \hline
% Downlink bandwidth       & 200 Mbps~\cite{dove-uplink-downlink}                           \\ \hline
% On-board storage         & \textit{30 GB minimum}\footnote{This estimate is based on the absence of public data. Given a 200 Mbps download rate over 10 minutes, the satellite can download 15 GB. This data remains on-board until the next ground contact to ensure successful cloud storage transfer, totalling 30 GB. This is a conservative estimate, not favoring our proposal to store reference images on-board.}             \\ \hline
% On-board CPU             & \textit{EDGE 1U processor}~\cite{satellite-edge-cpu} \\ \hline
% Computation time per image   & \textit{22 seconds}~\cite{kodan}                \\ \hline
% Image resolution      & 6600$\times$4400~\cite{planet-ground-sampling-distance}                          \\ \hline
% Image channels      & RGB + InfraRed~\cite{planet-ground-sampling-distance}                          \\ \hline
% Image file size      & \textit{150 MB}~\cite{planet-image-size}                          \\ \hline
% Ground sampling distance & 3.7 meters~\cite{planet-ground-sampling-distance}                         \\ \hline
% \end{tabular}

% \end{table}


% \kt{Incorporate more latest work, cite more papers even if they are not directly related.}
% \kt{Change cloud removal to Kodan}

% \kt{Highlight that this downlink bandwidth is averaged across ground contact time}
\mypara{Optimization objective}
We aim to address the downlink bottleneck of satellite constellations by better {\em satellite image compression}.
% improving the \textit{image compression} step.
More specifically, we aim to use much less bandwidth to download the same amount of satellite imagery, measured in the number of photoed locations and frequencies, without compromising image quality.
% \jc{can we claim we don't compromise quality on all channels? otherwise, it may seem like we can trade one band's quality for another?}
% reduce the downlink bandwidth required to download the same number of images as existing satellites without compromising image quality.
To measure the quality of the downloaded images, we use Peak Signal-to-Noise Ratio (PSNR for short), which aligns with satellite imagery compression literature~\cite{indradjad2019comparison,gunasheela2018satellite,faria2012performance,shihab2017enhancement}.
% \jc{just to confirm: is your definition of PSNR the same as traditional BGR pixels? i thought you at least have more channels, etc. if there's any difference, please explain it here.}
% \kt{For me PSNR is agnostic to the number of channels or the bit depth. Claiming them here makes people feel that these characteristics change the meaning of PSNR, while they do not.}


% \kt{Highlight that we stick to real-world storage/uplink constraints, and do not use more computation than baselines.}
\mypara{On-board constraints}
While optimizing for the image quality and reducing the downlink consumption, we stick to real-world on-board storage, computation, and uplink constraints. 
We describe the real-world satellite specification that we used for our evaluation in \S\ref{sec:evaluation}.
% Here we assume that the uplink bandwidth is a constant, since the uplink leverages S-band~\cite{Sentinel-2-uplink}, where the attenuation caused by weather (\eg rain and snow) is negligible~\cite{s-band-rain}.


% \mypara{PSNR in satellite imagery}
% Compared to PSNR in traditional 
% \kt{Agree that we need to have some text on this.I'll focus on this part later since there is no fundamental difference between PSNR of traditional RGB images and satellite imagery (though there are some differences like multi-channel and high bit depth that does somehow change how people should interpret different PSNR values)}



% \jc{as part of the objective, please also explain what the constraints are and what the tunable parameters are. }
% \kt{Agree. Will do it after finishing technical section.}





%  as it correlates to the perfo-boardr, which reqmance of a wide range of satellite imagery applications like autonomous road detection~\cite{??,??} and forest detection~\cite{??,??}, etc.


% To make the discussion more concrete, we further characterize the resources constraints on a single satellite.
% We use the DOVEs constellation from Planet~\cite{planet} as an example.
% Note that we align the number to a time-frame from year 2017 to year 2018 for consistency.
% Table~\ref{tab:hardware-specs} for the concrete technical specs.
% Note that some of the data are not publicly available and we infer using other sources.

% Specifically, we aim to improve the quality of downloaded images (quantified by Peak Signal-to-Noise Ratio, or PSNR) and the volume of images downloaded per ground contact, all within the satellite's resource constraints. Using the DOVEs constellation from Planet~\cite{planet} as a reference, based on 2017 public data, the satellite constraints are:
% \begin{packeditemize}
% \item Downlink: 200 Mbps~\cite{dove-uplink-downlink}.
% \item Uplink: 250 kbps~\cite{dove-uplink-downlink}.
% \item Ground contact duration: 10 minutes~\cite{leoconn}.
% \item Estimated on-board storage: Minimum 45 GB\footnote{This estimate is based on the absence of public data. Given a 200 Mbps download rate over 10 minutes, the satellite can download 15 GB. This data remains on-board until the next ground contact to ensure successful cloud storage transfer. An additional 15 GB is reserved for potential ground disconnections, totaling 45 GB. This is a conservative estimate, not favoring our proposal to store reference images on-board.}.
% \item Image processing time: 22 seconds per image~\cite{kodan}, with each image sized 6600$\times$4400~\cite{dove-image-shape} and featuring RGB and InfraRed bands.
% \item Estimated computation hardware: EDGE 1U payload processor @2GHz~\cite{satellite-edge-cpu}.
% \end{packeditemize}




% The focus of this work is to enable better on-board image compression for general-purpose satellites.
% By enhancing compression techniques, we strive to download images for more geographical locations with higher frequency without sacrificing the quality of the downloaded image.

% Formally, we aim to optimizing the trade-off between quality of the downloaded image (measured by Peak Signal-to-Noise Ratio, PSNR for short) and the number of images downloaded during each ground contact, while adhering to the resource constraints on the satellite.
% To specify the constraints on the satellite, we use DOVEs constellation from Planet~\cite{planet} as the target scenario, using public information available at year 2017:
% \begin{packeditemize}
%     \item Downlink: 200 Mbps~\cite{dove-uplink-downlink}.
%     \item Uplink: 250 kbps~\cite{dove-uplink-downlink}.
%     \item Ground contact duration: 10 minutes~\cite{leoconn}.
%     \item Estimated on-board storage: 45 GB minimum\footnote{We estimate the on-board storage as there is no public data available. The ground station can download 200 Mbps$\times$10 minues=15 GB data from the satellite. After downloading, the satellite still needs to store the data on-board till next ground contact to make sure the data is successfully streamed to the cloud storage. Also, the satellite needs to further reserve 15 GB to handle one-time ground disconnection, resulting in a total of 45 GB. Note that this is a conservative estimation, which is not in the favor of our proposal of storing reference images on-board.}.
%     \item Computation deadline per image: 22 seconds~\cite{kodan}, where each image is of shape 6600$\times$4400~\cite{dove-image-shape}, with RGB and InfraRed bands.
%     \item Estimated computation hardware: low-end commercial satellite processor (EDGE 1U payload processor @2GHz~\cite{satellite-edge-cpu}).
% \end{packeditemize}



\tightsubsection{Existing solutions}

% \jc{shouldn't the subsec title be existing solutions?}

% To provide high-resolution satellite imagery with high frequency, more and more large-scale LEO satellite (low earth orbit) constellations are developed for earth observation purpose in recent 5-10 years.
% For example, Planet's DOVEs constellation contains about 130 satellites that provide high-resolution satellite imagery (with a GSD of 3m) every day.

% We want to point out three characteristics of recent LEO satellite constellations:
% \begin{packeditemize}
%     \item \textbf{\textit{Large constellation size}}: Recent LEO satellite constellations (\eg DOVEs constellation~\cite{planet} and Lemur-2 constellation~\cite{lemur2}) contain more than 100 satellites.
%     \item \textbf{\textit{High-resolution imagery}}: These satellite constellations provide much higher resolution imagery (\eg 3-meter GSD in DOVEs constellation~\cite{dove-constellation}), where traditional satellites typically has much lower resolution (\eg 250-meter GSD in MODIS~\cite{MODIS}).
%     \item \textbf{\textit{High ground access frequency}}: Due to the large constellation size, these constellation can photo the earth frequently (\eg daily in DOVEs constellation~\cite{planet}).
%     \item \textbf{\textit{Downlink-heavy connectivity}}: LEO satellites have high downlink capacity (\eg 200 Mbps for DOVEs constellation at year 2017~\cite{dove-uplink-downlink}) but limited uplink capacity (\eg 250 kbps in DOVEs constellation~\cite{dove-uplink-downlink}).
%     Moreover, earth-observation LEO satellites typically do \textbf{\textit{not}} have inter-satellite connections.
% \end{packeditemize}


There are several approaches to addressing the downlink bandwidth bottleneck.


\mypara{Upgrading infrastructures}
The first is to physically increase the total downlink capacity of the satellite constellation by upgrading the infrastructure (\eg building more ground stations~\cite{planet} or adding more satellites~\cite{planet,sentinel-2,kodan}).
The costs of such infrastructure changes can be prohibitive, and they can be slow. For example, it takes tens of millions of dollars to build and send just one single satellite~\cite{satellite-cost}.

\mypara{On-board filtering}
An alternative is to filter the imagery onboard the satellite~\cite{kodan,serval,oec}.
For the mission-specific constellations that focus on specific regions, this approach can filter out most of the imagery.
For instance, the Biomass mission targets forest areas to monitor forest coverage changes~\cite{biomass}, while the IceBridge mission observes polar ice to gauge climate change impacts~\cite{icebridge}. 
However, 
%while the downlink capacity of these constellations suffices to download their respective regions of interest, 
they must exclude data useful for other applications. For example, the Biomass mission omits about 91\% of the Earth's surface~\cite{forest-area,ocean-area}, such as city areas (which are useful for smart city applications) and agriculture areas (useful for digital agriculture).

\mypara{In-space application processing}
% \edit{This addresses reviewer B's comments on related work}{
Instead of downloading the imagery to the ground, a wide range of systems process the application onboard the satellite and stream the application results back to the ground~\cite{inspace3,inspace1,inspace2}.
However, this approach cannot support many applications due to limited on-board compute, while downloading imagery to the ground allows all applications to perform analytics based on downloaded imagery.
% }



\mypara{Inter-satellite link for multi-path imagery delivery} \\
% \edit{This put the coherent optical communication works mentioned by reviewer B into context}{
Boosted by coherent optical communication~\cite{coherent-1,coherent-2,coherent-3}, the inter-satellite link capacity is quickly growing and allows multipath satellite imagery delivery that can significantly reduce imagery delivery latency~\cite{falcon,orbitcast}.
However, this approach does not increase the total downlink capacity of the satellite constellation, or reduce the total amount of imagery data that need to be downloaded, so it is still bottlenecked by limited downlink capacity.
% }

\mypara{On-board satellite imagery compression}
This work focuses on onboard imagery compression, which is complementary to the first three approaches. 
Existing solutions include augmenting single-image codecs~\cite{edge-prediction,progressive-jpeg2000,CALIC,linear-prediction,band-reordering,band-reordering-segmentation,band-reordering-prediction,band-prediction} and developing more expensive neural-based codecs such as autoencoders~\cite{autoencoder-1,autoencoder-2,autoencoder-3,autoencoder-4,autoencoder-5}.
However, these techniques focus on compressing single imagery from a single satellite, so they fall short in leveraging the {\em redundancies between} images for higher compression efficiency.


%There is another line of work that performs onboard satellite imagery compression (\eg augmenting existing codecs~\cite{edge-prediction,progressive-jpeg2000,CALIC,linear-prediction,band-reordering,band-reordering-segmentation,band-reordering-prediction,band-prediction} and developing neural-based codecs such as autoencoders~\cite{autoencoder-1,autoencoder-2,autoencoder-3,autoencoder-4,autoencoder-5}).
%However, this approach focuses on compressing single imagery and thus falls short in leveraging the redundancy \textit{between} images to provide further compression.
%
%We highlight that such limitation (\ie not leveraging the redundancy between images for better compression) is a common limitation across all three approaches.



% For those general-purpose satellite constellations (\textit{e.g.} Planet~\cite{planet}, Sentinel-2~\cite{sentinel-2}, MODIS~\cite{MODIS}), they handle the downlink bottleneck by either lowering the resolution of the imagery
% These satellite constellations handle the downlink bottleneck in two different ways.
% \begin{packeditemize}
%     \item One approach is to lower the image resolution.
%     For example, in MODIS~\cite{MODIS} constellation, each satellite captures images with a ground sample distance (defined as the geographical distance between the center of two nearby pixels, GSD in short) of 250m.
%     This resolution, however, falls short for tasks like crop monitoring or urban expansion analysis, which demand a GSD between 5-30m~\cite{application-GSD}, or 3D city monitoring and precision agriculture, requiring a GSD of 1-5m~\cite{application-GSD}.
%     % \jc{can we briefly mention some other whole-image compression works and say they are not much better because all pixels have to be compressed?}
%     % \kt{done}
%     \item Another approach is to augment the total downlink capacity by building more ground stations~\cite{planet} to increase the time of ground contact or adding more satellites to parallel the downloading between multiple satellites~\cite{planet,sentinel-2,kodan}. 
%     This approach can be prohibitively expensive and slow: it takes hundreds of millions of dollars to build and send just one single satellite~\cite{satellite-cost}. 
%     % Despite such investment, a substantial portion of images, such as ocean areas for Sentinel-2~\cite{sentinel-2}, still remains undownloaded.
% \end{packeditemize}



% In parallel, prior work also improves image compression by augmenting traditional image codecs like JPEG-2000~\cite{edge-prediction,progressive-jpeg2000,CALIC,linear-prediction,band-reordering,band-reordering-segmentation,band-reordering-prediction,band-prediction} or developing neural-based codec such as autoencoders~\cite{autoencoder-1,autoencoder-2,autoencoder-3,autoencoder-4,autoencoder-5}.
% % However, the improvement of this approach is marginal, as it compresses all pixels in the satellite imagery.
% \kt{I edited the following sentence. Does this sound OK?}
% However, this approach focusing on compressing a single imagery, thus falls short in leveraging the redundancy \textit{between} images to provide further compression.
% % While satellite imagery remains largely unchanged between two consecutive captures of the same location.





% \section{A seemingly promising approach: \\Change-based encoding}

% \jc{after skimming the early sections, i feel maybe it's better to shorten section 3 and merge it with section 4 greatly. here's an alternative flow:
% \begin{packeditemize}
% \item we start by saying we use change-based encoding, which hasn't received much attention since using reference images locally can easily be stale, and consequently, most regions will be downloaded anyway (mention the paper that uses fixed ref images). 
% \item then back this argument up with something like figure 3.
% \item briefly mention that even if a satellite updates the ref locally, the gap between two usable images can sometimes be too big. (this part should focus on why one satellite can't visit a location too frequently. otherwise, it should be brief.)
% \item bring up the constellation-wide solution
% \end{packeditemize}
% }

% \kt{Sure, now working on this flow.}




% Next, we introduce change-based encoding, a seemingly promising idea that leverages history images to pinpoint regions that have recently changed. 
% As we will see, directly applying this approach does not work well as history images locally available to each satellite are not fresh enough to unleash the benefit of change-based encoding. 
% % and point out the benefit of up-to-date reference images on change-based encoding. We then show that satellite imagery captured from one single satellite is not up-to-date enough.



% % \subsection{Compression potential}

% % \subsection{Detecting changes based on history images}
% \subsection{Why change-based encoding?}
% \label{subsec:up-to-date-reference}

% \kt{This need some further details}
% Previous efforts have shown that the geographical content in satellite imagery remains largely the same or changes slowly compared to the recent image that captures the same area~\cite{satroi,virtual-background}.
% As a result, one can use the latest image captured in the same area as \textit{reference}, which we refer to as the \textit{reference image}.
% Using the reference images, the satellite can pinpoint the areas that have changed after the reference image was taken and only compress and transmit the changed areas.
% % need to be transmitted to the ground.
% Leveraging this insight, a recent change-based technique shows that 
% % to substantial compression of satellite imagery, achieving 
% up-to 4$\times$ more efficient compression on cloud-free images~\cite{satroi} than encoding the images in their entirety.
% % \jc{in the last claim, shouldn't there be a caveat that the reference image be within \fillme hours apart from the current image? i understand you will bring this up immediately in the next para, but please remember that people may stop reading at any point.}
% % \kt{I choose not to spell the frequency of updating reference here as it invites more questions. If the reference is refreshed once every 4 days, people may think that you are already refreshing image frequently but the gain is still only 4x, which sounds marginal. And why cannot your approach achieve 4x gain?}





% % \subsection{Key: up-to-date reference image}


% A key factor influencing the compression ratio in change-based encoding is the staleness of the reference image, where we define {\em staleness} as the time gap
% between the reference image and the current observed image.
% The smaller this time gap, the less change happened in the observed image compared to the reference, meaning less change needs to be downloaded and thus less downlink usage.


% To measure the effect of the staleness on change-based encoding, we use 1-year cloud-free images over 9 locations (each location is of size 1600 $km^2$) sampled from Washington State and measure the (averaged) percentage of changed areas under reference images with different staleness.
% We define changed areas as those with pixel value differences over 0.01\footnote{This pixel difference threshold roughly translates to PSNR over 38db, which means those areas deemed ``unchanged'' would still have a high PSNR (quality) by simply reusing the pixels in the reference image.} compared to the reference image.
% Here, the pixel differences are computed after we normalize pixel values to [0,1] and align the illumination between the image and its reference (\S\ref{sec:dynamism}).
% % \footnote{Note that we normalize the pixel value to [0, 1] and then calculate pixel value difference. We also align the illumination between the image and its reference before calculating the pixel difference.\jc{can we cite something here and say we follow the common practice?}}.
% % \jc{can we put 0.01 in perspective? is 0.01 typically used by prior work to determine whether a region has enough change and needs to be updated?}
% % \kt{This part is much more nuanced than I initially thought. The target of traditional change detection is to fit human ground truth, and on the algorithm side, the corresponding change detection threshold is set adaptively. 
% % But in our scenario, the change detection is to improve PSNR, which is much easier cuz PSNR is agnostic to video content and is only sensitive to large pixel differences, so thresholding is a natural choice.}



% Figure~\ref{fig:staleness-change} shows that the percentage of changed areas (Y-axis) grows with the staleness of the reference image (X-axis).
% % \kt{I feel like explaining the reason of why this curve is not monotonic (which is because for certain staleness the number of image pairs is only 5 pairs and thus have statistic noise) may invite questions like why don't you collect more images.}
% % \footnote{Note that the percentage of changed area does not strictly grow with the staleness of reference image, as we gather the satellite revisits the ground at roughly once per 10 days, so the , there may not be sufficient}. 
% % \mypara{Measurement highlight}
% For example, {\em the changed areas will drop by \textbf{half} if we reduce the staleness of reference images from 30 days to 10 days}.
% This suggests that we can further save up to 2$\times$ downlink bandwidth if we reduce the staleness of the reference image from 30 days to 10 days.
% % \jc{this last sentence needs to be highlighted! and please refer to it in later sections: whenever a method reduces the staleness by 3x or something, we should always remind people what that means to the areas to be downlowded}

% % This indicates that: reducing the staleness of the reference image allows the satellite to download less changed areas, and thus reducing the total downlink demand.

% \begin{figure}[t!]
%     \includegraphics*[width=1\columnwidth]{figures/staleness-change.pdf}
%     \caption{More changes must be downloaded if the reference image is stale. \jc{smoother + drop below 10}}
%     \label{fig:staleness-change}
% \end{figure}



% % \begin{figure}[t!]
% %     \includegraphics*[width=1\columnwidth]{figures/staleness_planet_measurement.pdf}
% %     \caption{By gathering reference images from the whole constellation (``Constellation-wide''), one can reduce the staleness of reference images by 30$\times$ compared to seeking reference images based on historical images captured by the same satellite (``Satellite-local'').}
% %     \label{fig:staleness-change}
% % \end{figure}



% % As shown the changed areas as those pixels that have in Washington area using Sentinel-2 dataset, and found that the average amount of changes reduced by half if the freshness of reference images went down from 10 days to 5 days. \kt{need to expand this experiment in detail}




% % \jc{i understand the point of the next two paragraphs, but can we move it later. iiuc, the key point of 2.4 is that FRESH ref images can go a long way, but local ref images can be too stale. so just use that flow directly}





% % \begin{figure}[ht]
% %     \includegraphics[width=.99\columnwidth]{figures/dynamism.pdf}
% %     \caption{Two consecutively-captured satellite imagery have similar content on the ground but can significantly differs in terms of pixel value due to cloud and illumination difference.}
% %     \label{fig:satellite-imagery-dynamism}
% % \end{figure}
    

% % The first line of work uses video codecs to encode the changes (\eg H.264~\cite{h264}), with the assumption that two consecutive frames captured from one location have a small pixel value difference.
% % However, this assumption does not hold in the satellite imagery scenario since two consecutively-captured satellite imagery can still differ a lot due to cloud and illumination differences.
% % We illustrate the impact of illumination and cloud on satellite imagery in Figure~\ref{fig:satellite-imagery-dynamism}.
% % In this Figure, we show two consecutively captured satellite imagery, where the geographical content on the ground is almost the same but the pixel value highly differs due to cloud and illumination differences.

% % \subsection{Local images on the satellite are not fresh}
% \subsection{Why not {\em local} change-based encoding?}

% As a first attempt to apply change-based encoding to on-board satellite image compression, 
% % In order to maintain up-to-date reference images, 
% a simple design would use the latest image observed by the satellite at the same location as the reference. 
% We call this approach \textit{\textbf{satellite-local}} design.

% % Prior work developed change-based encoding in satellite imagery~\cite{satroi,virtual-background}.
% % This work successfully handles varying illumination and cloud conditions by illumination alignment and cloud removal~\cite{satroi,virtual-background}.
% However, such an intuitive design fails to obtain fresh enough reference images.
% This is because the satellite-local design only leverages \textit{local} images captured by the satellite to update the reference images on-board.
% % This makes the staleness of reference images being more than ?? days in average, forcing the satellite to download ??\% areas as change.
% % h may result in the staleness of reference images being more than ?? days and forcing the satellite to download ??\% changes.
% In constellation \fillme, each satellite takes an image at the same location every ten days~\cite{sentinel-2-revisit}, so the the latest locally accessible image will be ten days old.
% \jc{maybe add another satellite constellation? also explain why the revisit by the same satellite has to have such a long gap? is it inherent to the earth orbit or something?}
% % the local image for the same location is at least ten days ago since a single satellite retakes the image at the same location once every ten days~\cite{sentinel-2-revisit}.
% % This will work well if the reference images from 10 days ago are always cloud-free (as in the setup of Figure~\ref{fig:staleness-change}).
% To make it worse, the reference images can sometimes be partially covered by clouds, and those cloudy regions will not be useful as a reference anymore.
% In fact, it is shown that 67\% of the earth's surface is covered by cloud in average~\cite{cloud-coverage}, so the captured images are likely at least partially covered by clouds.
% In those cases, the satellite must search further in history to find a cloud-free reference, which increases the staleness to 20 days, 30 days, or higher. 

% % Moreover, in the case that the image observed 10 days ago may be fully cloudy and cannot be used as a reference, and most of the images cannot be used as reference images as they may be cloudy\footnote{Note that about 67\% of the earth surface is covered by cloud in average~\cite{cloud-coverage}, so it is likely that the images captured is cloudy.}.
% % In practice, the staleness of the reference image is much higher than 10 days, as the reference image needs to be cloud-free, while the probability of capturing a cloud-free image is only 33\% on average since 67\% of the earth surface is covered by cloud in average~\cite{cloud-coverage}.
% % \jc{please make it concrete. i understand why you said it could be more than 10 days, but can you make it more concrete. on average, 15 days? 30 days? or 50 days? maybe show a CDF of the distribution of the staleness in our dataset? btw, 10 days is on the low end from fig 2, so you really need evidence to convince people that the staleness is often close to 50 days or more.}

% \kt{I will redo this measurement on more locations, so skip this paragraph for now.}
% To further quantify the staleness of reference images, we measure the staleness of reference images on an agricultural location in Washington (10TES in military coding) in the year 2020, using the images from one single satellite (S2A satellite from Sentinel-2~\cite{sentinel-2-revisit}).
% We show that the staleness of reference images can be over 40 days if using images from one single satellite, resulting in more than 30\% of the changed areas needing to be downloaded.



% % However, existing work fall short on this front since it only relies on the local images available on the satellite to reduce the staleness of reference images.
% % However, as the satellite revisits a location once per 10 days~\cite{sentinel-2-revisit}, the reference image can only be refreshed at most once per 10 days, 
% % Existing methods rely on the satellite itself for reference image updates. 
% % Given that a satellite revisits a location approximately every 10 days~\cite{sentinel-2-revisit}, on-board reference images can only be refreshed at this frequency. This leads to a minimum staleness of 10 days, which can extend further if the observed image is clouded and cannot be used to update the references.

% % \mypara{Challenge}
% % As a result, the challenge of such change-based encoding is how to obtain reference images on-board.
% % Facing this question, prior work use the satellite itself to update the reference images.
% % As the satellite revisits one location once every 10 days~\cite{sentinel-2-revisit}, the reference images on-board can only be updated once every 10 days, resulting in a staleness of at least 10 days (the staleness will be more than 10 days if the observed image is cloudy and cannot be used to update the reference).

% % First, due to limited storage capacity on the satellite, these reference images need to be compressed for more than 200x\kt{200x is a placeholder number}, which makes change-based encoding no longer useful.
% % To quantify how much the compression of reference images hurt the performance of change-based encoding, \kt{fill in the concrete setup here}.
% % From the figure, we can see that when the reference images are compressed by >200x, more than half of the geographical areas need to be downloaded  even when the actual change is less than 5\%.



% % A critical challenge emerges when considering the practical implementation of change-based encoding for on-board compression. An in-depth analysis reveals that to fit within the satellite's limited on-board storage capacity, reference images must undergo compression exceeding a factor of 200x. This compression threshold presents a significant hurdle as it substantially diminishes the potential benefits of change-based encoding.

% % Experimental Validation

% % To quantitatively assess the impact of compressing reference images by over 200x, a comprehensive measurement experiment is conducted. This experiment employs a dataset sourced from the Sentinel-2 satellite, focusing on image pairs that meet specific criteria: cloud-free conditions and a time interval of no more than 10 days between captures (matching the Sentinel-2 revisit time).

% % The experiment yields illuminating results, with the compression ratio of the reference image plotted along the X-axis and the percentage of areas requiring downloading to cover 99\% of changes plotted along the Y-axis. A key takeaway from this experiment is that the potential efficacy of change-based encoding is significantly curtailed when the reference images are subjected to compression beyond a factor of 100x.

% % A Novel Design Approach

% % In light of these findings, we advocate for a fresh design paradigm. Our proposal involves a strategy where the satellite retains reference images for a select subset of locations. To ensure the most up-to-date reference images, the ground-based stations periodically update these references via uplink communication.

% % By adopting this innovative approach, we aim to strike a balance between efficient compression and accurate representation, thereby optimizing the utility of satellite imagery within the constraints of a general-purpose satellite system. Through this avenue, we aspire to enhance data retrieval frequency and alleviate the financial pressures associated with expanding downlink capacity for future satellite systems.


% % \subsection{Earth observation satellites}

% % Satellite imagery is serving applications that are used in our daily life. 
% % For example, satellite imagery can be used to detect roads automatically, learn the forest conditions and monitor agricultural areas.


% % As a result, a lot of earth observation satellites are sent to observe 

% % However, satellites are now generating much more data than the downlink can afford.
% % For example, a Sentinel-2 satellite generates 1.6 TB~\cite{sentinel-data-generation-rate} data per day.
% % But the downlink capacity is only 0.3 TB per day on average\footnote{The connection between the satellite and the ground happens 6-8 times per day, and each time the contact lasts between 5 to 15 minutes~\cite{satellite-ground-contact-time}. The downlink bandwidth of such a connection is 560Mbps~\cite{sentinel-data-generation-rate}, resulting in a daily downlink capacity of 0.3TB on average}, 5x smaller than the daily generated data.
% % The gap between the daily generated data and daily downlink capacity will be even larger if the ground-satellite connection is partially blocked by the cloud.

% % As a result, we desire a compression algorithm on the satellite that can significantly reduce the amount of data need to be downloaded while still maintaining high image quality.



% % % \begin{itemize}
% % %     \item daily data generated = ??TB << daily downloaded data = ?? TB, references
% % % \end{itemize}

% % % \subsection{Potential of on-board change-based compression}

% % % \begin{itemize}

% % The opportunity is that: most of the geographical areas do not change between two consecutive satellite visits and thus do not need to be downloaded.
% % In other word, the satellite only need to download those areas that are changed, we call this approach \textit{change-based encoding}.

% % To measure the compression potential of change-based encoding, \kt{State the setup of measurement experiment}. We found that only 5\% areas are changed and need to be downloaded in over 95\% of captured satellite images, where we define those areas that need to be downloaded as their PSNR will drop below 35 if not downloaded properly.
% %     % \item A measurement using PlanetScope dataset, a figure like ~\ref{fig:unchanged_areas}.
% %     % \item Ideally get some citations to support this point.
% % % \end{itemize}
% % \jc{i like this point, but i suspect it's not the first time people observe that satellite images change slowly. any prior work we can cite? and did they also define change as delta in PSNR (which seems a bit arbitrary)? }
% % \kt{roger, let me do some literature search}



% % However, the key design question of such change-based encoding is: how to obtain a reference image for \textit{all} geographical locations \textit{on the satellite}.

% % A simple solution is to let the satellite store reference images for all geographical locations, and the satellite use the newly captured image to update its reference image.

% % However, this approach only leverages resources on the satellite, which is limited and not sufficient to accurately detect changes due to the following three reasons: 
% % \begin{packeditemize}
% % \item First, the storage on the satellite is not sufficient to store the reference images for all geographical locations.
% % Take Sentinel-2 satellite~\cite{sentinel-data-generation-rate} as an example. 
% % As Sentinel-2 satellite visit every geographical location on the earth every 10 days, the satellite needs to store 10 days worth of data in order to make sure the newly visited location has a reference image from last visit.
% % This requires an \textit{extra} 16TB storage on the satellite.
% % This number is 50x larger than the disk size of the current satellite, which is 0.3 TB~\cite{sentinel-data-generation-rate}.
% % \item \kt{here} Second drawback is that this solution updates the reference image at a low frequency (about once per 10 days). A lot of changes can happen in 10 days, and this significantly reduces the change. 
% % An example: harvesting seasons, 10 days, ??$km^2$ areas are harvested
% % \end{packeditemize}


% % \begin{figure}
% % \includegraphics[width=1\columnwidth]{figures/storage-vs-downlink.jpg}
% % \caption{Storage v.s. daily generated data between different solutions}
% % \label{fig:storage-vs-downlink}
% % \end{figure}


% % \begin{figure}
% % \includegraphics[width=1\columnwidth]{figures/multi-satellite-as-reference.jpg}
% % \caption{2x less changed areas when using images from 2 satellites as reference.}
% % \label{fig:multi-satellite-as-reference}
% % \end{figure}




% % \subsection{Uplink-based}



% % We propose a new \textit{uplink-based} design: the ground let the satellite store a small subset of reference images, and use the \textit{uplink} to \textit{update} this subset of reference image.
% % \jc{we should emphasize that this "small subset" only needs to contain ref images for locations to be visited before the next ground-station fly-by. is it correct?}

% % \jc{there seems an implicit assumption that this "small subset" is small enough to fit the on-board storage. is this obvious? (at least not to me)}

% % \kt{Ideally ?? areas, if the uplink is 2x worth ==> 2x more areas stored}

% % The advantage of this uplink-based design is two-fold.


% % First, it significantly reduces the storage demand on the satellite.
% % Need a calculation to show that if the uplink \textit{were} available everytime the satellite contacts the ground, the satellite only needs to save reference images for, say 1\% of the area.


% % Second, this design allows the satellite to asdf. virtually refer to the reference images from other satellites.


% % Third, the propagation delay is low. ground can update the reference image everytime the satellite contact the ground.
% % As the satellite contacts the ground once every 90 minutes in average, this design allows the satellite to frequently update the reference image.


% % A measurement figure (Figure~\ref{fig:multi-satellite-as-reference}): benchmarked on PlanetScope dataset, using uplink v.s. not using uplink ==> 10x less of changed areas.

% % \kt{Mention that why it is hard to detect changes}
% % \kt{Take a blank paper and write the pitch in bullet points, the intro and section should follow the flow, and we need to be able to substantiate each point}
% % \kt{Evaluation: evaluate the main claims in the introduction}



% % \begin{figure}
% % \includegraphics[width=1\columnwidth]{figures/single-vs-multi.jpg}
% % \caption{The satellite-only approach only uses images from itself. As a result, 5x more areas will be detected as changes compared to using the images from multiple satellites.}
% % \label{fig:single-vs-multi}
% % \end{figure}

% % \begin{figure}
% % \includegraphics[width=1\columnwidth]{figures/change-detection-accuracy.jpg}
% % \caption{The parameters of change-based detection need to be customized per-season per-location.}
% % \label{fig:change-detection-accuracy}
% % \end{figure}





==> tex-files/intro.tex <==
%!TEX root = ../paper.tex
%!TEX spellcheck = en_US


\section{Introduction}


Nowadays, people use large language models (LLMs) in more and more applications.
Besides the generative applications that generate new content for people to read and use, like chatting (\eg ChatGPT, Character.AI), code generation (\eg Github Copilot, Cursor) and search summarization (\eg Perplexity), 
researchers and practitioners have started to use LLMs to replace traditional deep learning models in applications such as recommendation, credit verification, and data labeling.

The reason behind this trend is two-fold: 
\begin{packeditemize}
    \item \textit{Streamline the development}: 
   Traditional deep learning pipelines often require multiple iterations of data preprocessing, feature engineering, and model tuning to improve performance. This is complex and time-consuming, as it typically involves cross-team collaboration.
    In contrast, LLM-based solutions can process raw text directly and are general enough to obviate finetuning. This allows developers to interactively debug and improve the pipeline by just changing the prompts. 
    \item \textit{Higher decision quality with comparable performance}: By properly selecting the size of the LLM model and engineering the prompt of LLM-based pipeline, the decision quality can be achieved compared to traditional deep learning pipelines with comparable performance.
\end{packeditemize}

\begin{figure}
    \centering
    \includegraphics[height=0.52\linewidth]{figures/contrast_traditional_prefill_only_traditional.pdf}
    \includegraphics[height=0.52\linewidth]{figures/contrast_traditional_prefill_only_prefill_only.pdf}
    \caption{Contrasting traditional LLM requests and prefill-only LLM requests. In prefill-only requests, the KV caches will not be immediately reused, and the output length is always 1.}
    \label{fig:contrast_traditional_prefill_only}
\end{figure}


Our insight is that in many of these applications, \textit{LLMs only generate one single output token for each incoming request}. 
This minimizes LLM generation latency while still allowing the LLM to express its preference towards multiple choices.
For example, in a document recommendation application, if we want to ask LLM whether we should recommend a document to a user, we can construct the following LLM query:
``\texttt{Here is the user profile: [user profile], and here is the document: [document]. Should we recommend this document to this user? Your answer is: }'',
and then determine whether the LLM thinks that we should recommend this document or not by constraining the choice of output token to only \texttt{Yes} and \texttt{No} and then observe the LLM output token.
See \S\ref{subsec:prefill-only-example} for more details.


%  and then observe the output probability distribution, \ie $P(\text{Output token is }\texttt{Yes})$ and $P(\text{Output token is }\texttt{No})$, where the sum of these two probabilities is 1.
% The recommendation application can then recommend the document with highest $P(\text{Output token is }\texttt{Yes})$.
% In other word, we observe two probabilities, where the  in other word, we only observe P(\texttt{Yes}) P(\texttt{No}).
% We then let LLM choose between ``Yes'' and ``No'' by letting LLM generate the output distribution on just two tokens, the ``Yes'' token and the ``No'' token in the vocabularity. 

% generate the distribution of the single output token,\textit{constraining} the selection of output token to only ``Yes'' and ``No'', and let LLM generate the output distribution of the 
% This allows people to the LLM to choose between options (\eg by )
%We identify a new workload behind such trend, in which \textit{LLMs only generate one single output token for each incoming request}.
% \ion{Most of the rest of this paragraph can be removed as it is repetitive. The one thing though to clarify is the "constraining the choice" part. Give an example.} This is because traditional applications are latency-sensitive, and generating just one single output token significantly reduces the latency of running one request, while still allowing LLMs to make decisions between multiple options (\S\ref{subsec:prefill-only-example}).
% Further, one can fully control the output behavior of LLM by simply constraining the choice of this single output token (while fully controlling the output behavior in traditional LLM workload remains challenging due to dependencies between output tokens).
% As a result, this approach builds a low-latency and robust foundation for people to build applications on top of LLMs.
% System-wise, the key characteristic of this workload is that it only requires running the prefilling stage of LLM inference.
% As a result, we name this workload \textit{prefill-only} workload. \lily{I feel it will be better to provide a concrete example here. For example, how is recommendation task formulated with LLM.}


From a system perspective, such workload only requires running the prefilling stage of LLM inference.
As a result, we name this workload \textit{prefill-only} workload.


To serve such prefill-only workload, we aim to build an LLM inference engine that minimizes the online serving latency without hurting the throughput.
% Hardware-wise, we focus on GPUs without hardware-accelerated inter-connections, as these GPUs are easier to maintain and more available in datacenter.
% \ion{This statement raises the question: are you actually focusing on these low end GPUs because your solution performs better on those GPUs? Keep in mind that Nvidia pushes people to use the high end GPUs for everything including inference. A better way to say it is that we provide significant performance improvements on all GPUs, and in particular on cheaper, reosurce constraint GPUs.} \lily{Another point, I guess workloads are generally running on low-end GPUs before LLM. So we just use the same GPU, replace the traditional model with LLM, that's why we run those models on low end GPUs. But agree with Ion, we should say it improves performance across all GPUs.}

We argue that existing LLM engines inflates the latency of prefill-only requests due to two reasons.

First, existing LLM engines fully cache the request state in GPU, which significantly reduces the latency for traditional generative request but actually does not reduce the latency for short request and inflates the latency of long requests in prefill-only request.
Concretely, for traditional generative request, fully caching the request state in GPU significantly reduces the delay of processing such request, because it requires multiple rounds of LLM inference (to generate multiple output tokens for this request) and caching the reqeust state accelerates the LLM inference from the second round.
However, for prefill-only request, fully caching the request state does not reduce the latency of this request, as it only requires one round of LLM inference. 
Further, it may inflate the latency when handling long requests, because fully caching the request state limits the longest requests that the LLM engine can handle (since the request state is large), and thus, when handling a request longer than the limit, the LLM engines have to either process the input chunked-by-chunk, which inflates the request latency, or parallel the inference, which incurs extra communication cost and may inflate the request latency especially when GPUs are not directly connected
via hardwares like NVLink.


A natural optimization for prefill-only workload is to \textit{discarding the request state}.
This is a widely adopted solution in traditional deep learning system literature.
However, this solution does not work well in LLM scenario due to two issues:
\begin{packeditemize}
    \item Future requests can reuse the request state to accelerate inference when they share the same prefix as the current request, and discarding the request state of current request prevents this acceleration.
    \item Discarding the request state only allows the LLM to process marginally longer request ($1.6\times$ as shown in \S\ref{??}) without chunking the request or parallelizing the inference.
\end{packeditemize}
To address these two issues, we proposes two novel techniques:
\begin{packeditemize}
    \item sdf
\end{packeditemize}



We argue that the latency of existing LLM engines manage are high when serving prefill-only workload.
This is because existing LLM inference engines are designed for multiround LLM inference, where some of the design choices improve multiround LLM inference at the cost of inflating the latency of the first round (\ie prefilling) and thus increases the latency of prefill-only requests.
Concretely, we characterize two design choices that inflates the latency of prefill-only requests:
\begin{packeditemize}
    \item \textit{Request state caching}: Existing LLM engines  fully cache the request state (in the format of KV caches or latent tensors) in GPU to accelerate the future round of LLM inference.
    However, such caching does not reduce the latency of prefill-only requests as they only requires one round of LLM inference.
    Further, the request state is large and fully caching it in GPU limits the longest requests the LLM engine can handle.
    Thus, when there are long requests in the workload, the LLM engines have to process the input chunked-by-chunk, which inflates the prefill latency, or parallel the inference, which incurs extra communication cost and may inflate the request latency, especially when GPUs are not directly connected via hardwares like NVLink.
    \item \textit{JCT-agnostic scheduling}: As the total rounds of LLM inference of one request depends on  number of output token, which is not fully predictable (and can even be non-deterministic) in traditional generative workload, existing LLM engine choose to use scheduling algorithms that are agnostic to job completion time (JCT), such as first-come-first-serve.
    However, in prefill-only workload, it just require one round of LLM inference to handle one request, and thus the JCT can be perfectly estimated.
\end{packeditemize}

% itself, but depends on 
% focus on optimizing decoding throughput, which the output generation throughput, in a way that inflates 
% significantly inflate the online serving latency for such prefill-only workload. 
% This is because existing LLM engines inherently assume that the requests need to go through multiple round of LLM inference to generate multiple output tokens, so that the scheduling should maintain states between requests.
% Based on this assumption, they assume that:
% \begin{packeditemize}
%     \item The request state (in the format of KV caches) needs to be cached inside GPU so that future requests can reuse.
%     \item 
% \end{packeditemize}
% assumption that  are optimized for the autoregressive generation case, where the requests need to be repeatedly inferenced  the LLM requests need multiple round of LLM inferences to generate m
% they are operate under the assumption that the requests are auto-regressive requests that require multiple steps of LLM inference.
% However, 
% engines are designed for auto-regressive requests, while 

% We found that the online serving latency of existing LLM engines is high because 


% The online serving latency of existing LLM engines is high due to two reasons: \zc{Fundamental diff: auto-regressive have complex dependency between steps, so you cannot discard KV cache and have to continue the running request. But we find prefill-only workload is simple, so we unlock more oppportunities, e.g., discard KV cache, more flexible scheduling algorithm.}
% \begin{packeditemize}
%     \item \textit{JCT-agnostic scheduling inflates latency}.
%     The scheduling algorithms of existing LLM engines are agnostic to job completion time (JCT), which inflate request latency compared to JCT-aware scheduling algorithms with perfect JCT estimation.
%     \item \textit{Handling long requests in a way that increases latency}.
%     LLM inference engines can only handle requests with limited input length, as GPU memory capacity is limited and can only store the KV caches (the key-value tensors of LLM's attention module, cached in GPU to accelerate LLM inference) for requests up to a certain length.
%     To handle requests longer than this limit, existing LLM engines must either process the request chunk-by-chunk (\ie chunked prefill), which allows handling upto 2$\times$ longer request but slows down the attention operation by 3$\times$, or increase the parallelism of the LLM inference engine, which incurs extra communication overhead and may result in higher latency when there is no hardware-accelerated inter-GPU connection available, or when the degree of parallelism is already large. See \S\ref{subsection:challenges} for more details.
% \end{packeditemize}


Thus, to reduce the latency of existing LLM engines on prefill-only workload, we propose two optimizations:
\begin{packeditemize}
    \item 
    \textit{Discarding request state}:
    As it only require one round of LLM inference to handle a prefill-only request, the request state does not need to be cached.
    \item
    \textit{JCT-aware scheduling}:
    In prefill-only workload, there is only one round of LLM inference per request, which makes the JCT fully predictable, allowing us to reduce request latency leveraging JCT-aware scheduling algorithms such as shortest-remaining-job-first.
    
\end{packeditemize}


Though these optimizations are not new and are widely used in  traditional deep learning serving systems \ion{some references}, 
we identify two practical challenges unique to the LLM workload:
\begin{packeditemize}
    \item Simply discarding the request state only allow the LLM engine to handle upto 1.6$\times$ longer requests, due to large intermediate tensors allocated by non-attention layers.
    \item As LLM engines may store the request state past requests \ion{previous words are confusing} to accelerate future requests that share the same prefix (also known as prefix caching), the JCT of one request changes over time, as the KV caches of new requests can evict those of older requests.
    \item Further, in the case when prefix caching is enabled, instead of fully discarding the request state for long requests, we should only partially discard the request state to maximize future reuse.
\end{packeditemize}

To address these challenges, we propose \name, the first LLM inference engine tailored for prefill-only workload.
\name proposes three novel techniques to overcome the aforementioned challenges:
\begin{packeditemize}
    \item \textit{Hybrid prefilling:} \name prefills non-attention layers chunk-by-chunk but prefills the attention layers normally.
    This reduces the GPU footprint of non-attention layers, enabling the engine to handle upto $7\times$ longer requests without inflating their latencies.
    \item \textit{Suffix request state discarding:} For long requests, \name stores the request state of as many \textit{prefix} tokens as possible in GPU, and discards the KV caches of remaining suffix tokens.
    This maximize the chance of prefix cache hit, while ensuring that caching behavior of \name only diverges with the traditional LLM engine when the request is too long for the KV caches to fully stored in GPU. 
    \item \textit{Continuous JCT calibration:} \name continuously calibrates the JCT of each LLM request based on current LLM engine's prefix cache, so that the scheduling algorithm can make decisions using accurate JCT estimates.
\end{packeditemize}

We implement \name on top of vLLM, a state-of-the-art LLM inference engine. We engineered \name so that it can generalize to different LLMs and hardwares without code modification, by implementing hybrid prefilling via \texttt{torch.compile}, and implementing suffix KV cache discarding without modifying hardware-related kernels.


We evaluate \name under different  hardware, LLM models and traces. Our evaluation shows that,  \name achieves 4$\times$ higher throughput without inflating the average latency compared to baselines, and can handle upto $7\times$ longer request without inflating the latency of that request.

To summarize, the contribution of this paper is as follows:
\begin{packeditemize}
    \item We identify a new trend in LLM use cases, where people use LLMs to substitute existing deep-learning-based pipelines, and characterize a new workload -- \textit{the prefill-only workload} -- that underlies these use cases.
    \item We propose \name, the first LLM inference engine tailored for prefill-only workloads, and show that it can significantly reduces latency compared to existing alternatives.
\end{packeditemize}


% \subsection{Old version}






% First, the maximum input length (MIL) that traditional LLM engines can handle is short (\S\ref{subsec:issues-of-limited-gpu-memory}), especially when handling large LLM models.
% %  on cheap hardware with limited GPU memory capacity .
% As a result, when handling requests with long input length, existing LLM engines have to either process the input chunk-by-chunk, which only increase the MIL by 2$\times$ at the cost of slowing down the attention operation, or spend extra communication to parallelize the inference, which can significantly increase MIL but hurts latency-throughput trade-off due to no high-speed interconnectivity between GPUs (see \S\ref{subsection:challenges} for more discussion).
% % parallel the inference, introducing extra communication overhead and 

% Second, existing LLM engines use JCT-agnostic scheduling algorithms like first-come-first-serve (FCFS).
% Though FCFS is starvation-free, it is agnostic to job completion time (JCT in short) and thus will have higher latency\lily{request latency?} compared to JCT-aware scheduling algorithms if we can provide accurate JCT prediction.


% % in order to generate multiple , and holding the KV cache in GPU significantly  holding the KV cache in GPU significantly accelerates the decoding phase of LLM.
% % However, this is not necessary for prefill-only workload, 
% % of all tokens and all layers in GPU.
% % Though this significantly accelerates the decoding phase of LLM, all KV caches in GPU caches the KV cache that is not reused.

% % First, traditional LLM engines hold all KV caches (the key-value tensors generated by the LLM attention layers) of one request in GPU when processing this request.
% % This significantly improves the output token generation throughput of LLMs (as the KV caches are reused repeatedly when the LLM generates the output tokens one-by-one) at the cost of having to run parallelization to handle long requests.
% % However, always storing all the KV caches of the request is not the best design choice in prefill-only workload, as it prevents LLM from serving longer request when the GPU memory capacity is limited, and it does not accelerate the processing of this request (as the KV caches are not reused during prefilling).

% Thus, to handle long-context requests with high throughput and schedule requests in a way that minimizes latency, we identify two unique opportunities in prefill-only workload:
% \begin{packeditemize}
%     \item \textit{KV Caching for computing layer only}: For prefill-only request, LLM engine only needs to  temporarily store the KV caches (intermediate tensors generated by attention layer) for just the computing layer, \ie the layer that is being inferenced, and the KV cache of all previous layers can be discarded.
%     This allow us to handle requests with long input length under the same GPU memory constraint without hurting the latency-throughput trade-off.
%     We not that this opportunity is unique in prefill-only workload: doing so in traditioanl LLM workload significantly inflates the request latency as discarding the KV caches prevents the LLM engine from saving the computation during decoding via reusing the KV caches, as shown in Figure~\ref{fig:contrast_traditional_prefill_only}.
%     % In contrast, caching for computing layer only does not increase the latency of processing prefill-only request, as the prefilling does not reuse the KV cache.
    
%     To put the potential of this opportunity into context, storing KV caches for only the computing layer allows us to handle upto number-of-LLM-layer-times longer request compared to storing the KV caches of all layers in GPU, which translates to 32$\times$ longer for popular LLM like Llama 3.1 8B.
    
%     \item \textit{Predictable JCT}:
%     As the output length of prefill-only requests are always one token, the JCT of these requests is fully deterministic and predictable. This allow us to leverage JCT-aware schdeduling algorithms to reduce the average latency and P99 latency of serving prefill-only requests.
% \end{packeditemize}

% % First, 

% % This type of workload presents two unique opportunities that is not typically presenting in traditional LLM workload.

% % Traditional LLM inference engines fall short to efficiently handle prefill-only workload, as there are unique optimization opportunities that are only applicable to prefill-only workload.
    
% % First, while traditional LLM need to cache the key-value tensors (KV tensors in short) for all LLM layers in GPU for future decoding, in prefill-only workload the engine only needs to store the the KV tensor for just one layer that is actively being inferenced (we denote such layer as \textit{active layer}).
% % By caching the KV tensors for just one layer, the LLM inference engine can handle upto number-of-layers-time longer input length, which translates to $32\times$ improvement in popular LLM models such as Llama 8B.

% % Second, while the job completion time (JCT in short) of traditional LLM requests cannot be accurately estimated (since the output length of LLM is not fully predictable), the JCT of prefill-only requests are fully predictable. 
% % This allow us to significantly reduce the average latency of prefill-only LLM requests by leveraging traditional scheduling algorithms like shortest-job-first scheduling, which yields upto ??$\times$ average JCT reduction compared to JCT-agnostic FIFO scheduling using recommendation production trace.

% % In short, these opportunity allow the LLM engine to improve context length by upto 32$\times$ and improve the average JCT by upto ??$\times$. 

% % Given this huge potential, the goal of this paper is to build an LLM inference engine tailored for prefill-only workload.

% However, it is challenging to realize aformentioned two optimization opportunities in practice.

% First, although storing KV caches for only one layer could theoretically increase the maximum input length (MIL) by $32\times$ for Llama 3.1 8B, naively doing so can only marginally improve MIL by $1.4 \times$.
% This is because the intermediate tensors allocated for non-attention layers becomes the major GPU memory bottleneck, as they are large (13$\times$ larger than the KV cache size of one layer) and linearly scales with respect to the input length.

% % We further discuss other solutions like chunked prefilling and parallelization-based solutions and show that they are also sub-optimal in \S\ref{subsection:challenges}.
% % We note that, the GPU memory footprint of these intermediate tensors can be controlled via processing the input chunk-by-chunk (also known as chunked prefilling). However, chunked prefilling slows down the attention operation, and can only marginally increase the context length (as it still requires storing the KV cache of all layers for previous chunks).

% Second, storing the KV cache of only one layer prevents the LLM engine from accelerating future requests via in-GPU prefix caching, a technique that accelerates future requests if they share the same prefix with previous requests and the KV caches of previous requests are cached in GPU.



% % our insight is that: the operations that introduce inter-token dependency (i.e. the attention operations) have negligible memory footprint.
% % Instead, the peak memory usage is mainly caused by the large intermediate tensors allocated by linear layers.
% % We examine that this phenomena widely exists in existing LLMs \kt{Need an empirical study to verify this.} for a good reason, as the key-value tensors are becoming more and more compact but LLMs have more and more parameters and thus LLMs needs to ``up-sample'' the compact key-value tensors in order to fully utilize the large amount of parameters.
% % \item This insight inspires us to process the attention operation for all input tokens and process the linear layers token chunk by token chunk.
% % This allow us to drop the key-value tensors generated by non-active layers while reducing the peak GPU memory usage.

% Third, traditional scheduling algorithms like shortest job first assumes that the JCT of each job roughly remains a constant.
% However, the JCT of each prefill-only request can vary significantly over time, because the JCT depends on not only the request itself but the in-GPU prefix cache inside the LLM engine as well, where the latter is constantly changing since new requests will bring in new prefix caches and evict old prefix caches.

% % To put the effect of varying JCT into context, we measure that, if we only estimate the JCT of each request once and perform simple shortest-job-first scheduling, the actual JCT of each request will differ by upto ??\%.
% % and thus makes the average latency ?$\times$ worse and makes the P99 latency ?$\times$ worse.

% To handle the challenges mentioned above, we present \name, the first LLM inference engine tailored for prefill-only workload.  
% \name proposes three novel techniques to address the three aforementioned challenges:
% \begin{itemize}
%     \item \textit{Hybrid prefilling:} \name prefills non-attention layers chunk-by-chunk but prefills the attention layers normally.
%     This allows \name to reduce the GPU footprint of non-attention layers without slowing down attention layers.
%     In addition, this technique allows \name to complete the prefilling in one forwarding pass, allowing \name to potentially discard the KV caches layer-by-layer.
%     \item \textit{Suffix KV cache discarding:} \name stores the KV cache of as many \textit{prefix} tokens as possible in GPU, and discard the KV caches of remaining suffix tokens.
%     We note that, this technique allows \name to benefit from prefix caching, and guarantees that the caching behavior of \name only differs with traditional LLM engine when the request is too long for traditional LLM engines to handle, \ie when the KV caches of this request cannot be fully stored in GPU. 
%     % the KV cache discarding mechanism to be non-intrusive: it only discards the KV cache when the request is too long to fully store its KV caches, so that \name can still 
%     % \name's optimization to be non-intrusive: it only discards the KV caches for those long requests with large amount of KV caches.
%     % This allows \name to fully leverage the benefit of in-GPU prefix caching, while still allow handling much longer requests by discarding the KV caches that cannot be stored in GPU.
%     \item \textit{Continuous JCT re-estimation:} \name continuously re-estimates the JCT of each LLM request based on current LLM engine's prefix cache, so that the scheduling algorithm can make decision based on accurate JCT.
% \end{itemize}

% % We note that hybrid prefilling will not change the LLM's inference results. 
% % This is because the non-attention layers are all linear layers in existing transformer-based LLMs, which means that there is no inter-dependencies between chunks and thus prefilling these layers chunk-by-chunk will not affect their inference results.
% % Also, though it is also possible to also prefill the attention layers chunk-by-chunk, \name choose not to do so.
% % The reason is two-fold:
% % \begin{itemize}
% %     \item Although prefilling attention layers chunk-by-chunk increases the context length, the improvement is marginal (only 1.6$\times$) it reduces the performance of attention operation. \kt{Need a mesurement here.}
% %     In contract, chunking the linear layers increases the context length the most (upto 14$\times$) without performance cost.
% %     \item Engineering-wise, there are tens of attention kernels for different hardwares, different quantizations and different use cases, and every attention kernel has different ways of preparing the input and thus require different chunking implementations.
% %     This is not a scalable effort.
% %     In contrast, chunking linear layers can be done transparently inside torch.compile without any code modifications to the model provider and the attention backend provider.
% % \end{itemize}

% We implement \name on top of vLLM, the state-of-the-art LLM inference engine.
% We highlight two implementation decisions of \name that allows \name to generalize to different LLM models and hardware.
% \begin{itemize}
%     \item Implement hybrid prefilling via \texttt{torch.compile}, which allows \name to perform hybrid prefilling without rewriting existing implementations of LLM models.
%     This allow \name to generalize to other models without code modification.
%     \item Implement suffix KV cache discarding without modifying hardware-related kernel codes, \eg the kernels for storing the KV caches.
%     This allows \name to generalize to different hardware without code modification.
% \end{itemize}

% We evaluate \name under different  hardware, LLM models and traces. Our evaluation shows that,  \name achieves \fillme$\times$ higher throughput without inflating the average latency compared to baselines, or reduces the average latency by \fillme$\times$ without reducing the throughput.
%     % \item The improvement of \name persists on \fillme different LLM models and \fillme different hardwares.
%     % without enlarge the maximum input length by 3.9$\times$, which allow \name to handle long-context request without using extra communication to parallelize the inference, leading to  \fillme$\times$ throughput improvement compared to parallelization-based solutions.
%     % \item \name reduces the average latency and P99 latency by \fillme$\times$ using continuous shortest job first scheduling.

% To summarize, the contribution of this paper is as follows:
% \begin{packeditemize}
%     \item Identify a new trend of LLM usecases, where LLMs are used to substitute traditional deep learning models, and a new trend of workload (the prefill-only workload) behind these usecases.
%     \item Propose \name, the first LLM inference engine just for prefill-only workload, and achieve 
% \end{packeditemize}

==> tex-files/intro_v1.tex <==
%!TEX root = ../paper.tex
%!TEX spellcheck = en_US


\section{Introduction}




Nowadays, large language models (LLMs) are widely used in generative applications.
%Besides the generative applications that generate new content for people to read and use, like chatting (\eg ChatGPT, Character.AI), code generation (\eg Github Copilot, Cursor) and search summarization (\eg Perplexity), 
% Besides the generative applications like
These include chatting (\eg ChatGPT~\cite{chatgpt}, Character.AI~\cite{characterai}), code generation (\eg Github Copilot~\cite{copilot}, Cursor~\cite{cursor}), and summarization (\eg Perplexity~\cite{perplexityai}) that generates new content for people to read and use.
However, researchers and industry practitioners have also started to use LLMs to replace traditional deep learning models in {\em discriminative} tasks, such as recommendation~\cite{firooz2025360brew,wang2023enhancing,wu2024survey}, credit verification~\cite{CatBoost,CALM,Vicuna}, and data labeling~\cite{Annollm,llmaaa,Doris}.
% \hejian{This also brings challenge to infrastructure support and maintenance debit.} \kt{Infra support and maintenance debit is the concrete difficulties of cross-team collaborations.}
The reason behind this trend is two-fold: 
\begin{packeditemize}
    \item \textit{Streamlining the development}: 
    Traditional deep learning pipelines often require multiple iterations of data pre-processing\cite{PreProAI}, feature engineering\cite{feature}, and model tuning\cite{modeltune} to improve performance. This is complex and time-consuming, as it typically involves cross-team collaboration. 
    In contrast, LLMs can process raw text directly and are general enough to obviate fine-tuning~\cite{firooz2025360brew,gpt3,limitedGenAI}. This allows developers to interactively debug and improve the pipeline by just changing the prompts. 
    \item \textit{Higher decision quality}: By properly selecting the size of the LLM model and engineering the prompt of the LLM-based pipeline, LLM can achieve comparable or higher decision quality compared to production models~\cite{firooz2025360brew}.
\end{packeditemize}

\begin{figure}
    \centering
    \begin{minipage}{1\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/contrast_traditional_prefill_only_traditional.pdf}
    \subcaption{Traditional generative LLM inference}
    \end{minipage}

    \begin{minipage}{0.8\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/contrast_traditional_prefill_only_prefill_only.pdf}
    \subcaption{Prefill-only LLM inference}
    \end{minipage}
    
    \tightcaption{Contrasting traditional LLM inference and prefill-only LLM inference. A prefill-only request does not have to reuse the KV cache for long decoding as it only generates one output token.}
    \label{fig:contrast_traditional_prefill_only}
\end{figure}


\mypara{Prefill-only workloads}
Our observation is that in many of these discriminative tasks, \textit{the LLM only generates one single output token for each incoming request}\cite{firooz2025360brew,llmrec,Doris,tallrec,fingpt,SMS}. 
% This minimizes LLM generation latency while still allowing the LLM to 
This is because a single-token output is sufficient to express the output of these tasks, \eg a preferred choice or a label.
%For example, in a document recommendation application, if we want to ask LLM whether we should recommend a document to a user, we can construct the following LLM query:
For example, the following prompt will be used in a document recommendation application:
``\texttt{Here is the user profile: [user profile], and here is the document: [document]. Should we recommend this document to this user? Your answer is: }''.
To determine whether this document should be recommended, the LLM only needs to generate one output token (\ie \texttt{Yes} or \texttt{No}).\footnote{To ensure that LLM only generates \texttt{Yes} or \texttt{No}, the developers do not have to fine-tune the LLM or add extra prompts; instead, they can pass a list of acceptable tokens (\eg \texttt{Yes} and \texttt{No}) to the LLM engine so that LLM engine only samples output from this list.
More discussion in \S\ref{subsec:prefill-only-characteristics}.}
%and then determine whether the LLM thinks that we should recommend this document or not by constraining the choice of output token to only \texttt{Yes} and \texttt{No} and then observe the LLM output token.
%See \S\ref{subsec:prefill-only-example} for more details.



% We identify two characteristics of this workload 
In this paper, we refer to such workload as \textit{prefill-only} workload, because
% From the perspective of the LLM inference engine, we identify two key characteristics of such workloads.
the LLM engine only returns one token, which only runs the prefilling stage of LLM inference.
% this workload only requires the LLM engine to execute the prefilling stage of LLM inference (as only one output token per request is required).
% Based on this, we name this workload \textit{prefill-only} workload.
Moreover, these prefill-only requests are often prefill-{\em heavy} since the input is typically long
% Also, we observe that the input length of these requests is typically long 
(\eg the user profile in the example above may contain months of user browsing history).
% such workload only requres running the prefilling stage of LLM inference such workload typically contains  only requires running the prefilling stage of LLM inference.




% \hh{Add 1 sentence here to say the latency is the optimization goal.}

Unfortunately, existing LLM engines use two particular design choices that are inefficient in prefill-only workloads. 

% of sub-optimal latency-throughput trade-off due to two design choices:
\begin{packeditemize}
\item {\em Massive request state in GPU memory:} Currently, LLM engines must store in GPU memory a large amount of KV caches or the latent tensors of attention layers, which we refer to as {\em request state}~\cite{PagedAttention,distserve,flexgen}. 
In a normal case, this state is repeatedly used to decode each output token, so storing the state significantly reduces the decoding delay. 
For prefill-only requests, however, this does not help, since the inference does not decode more than one token. 
In fact, caching the request state in GPU memory makes prefilling, particularly on long inputs, inefficient~\cite{aqua,loongserve}. 
Existing LLM engines leverage two solutions to fully store all KV caches, but both come at the cost of reduced throughput. Specifically, they either shard the request state across devices, incurring communication and synchronization overhead, or adopt chunked prefill, which lowers GPU kernel efficiency\cite{megatron,flexgen}.
    % \item \textit{Request state caching}: Existing LLM engines cache the request state of the incoming request (\ie the KV caches or the latent tensors of attention layers, we use request state for generality) in GPU.
    % Though caching the state of one request significantly reduces LLM inference latency of that request itself in traditional generative workload (since it accelerates the output generation starting from the second output token, as shown in Figure~\ref{fig:contrast_traditional_prefill_only}), it does not reduce the latency of that request in prefill-only workload.
    % Further, this caching hinders the capacity of LLM to handle long requests.
    % % This is a viable design choice in traditional generative workloads (which require multiple rounds of LLM inference to generate multiple output tokens), since caching the request state accelerates LLM inference starting from the second round, as shown in  
    % % as generative LLM request requires multiple rounds of inference to generate multiple output token, and caching the request state accelerates this request starting from the second round of LLM inference.
    % % However, caching does not reduce the latency of prefill-only requests because they only require one round of LLM inference.
    % As a result, the LLM engine must handle long requests either by processing the input chunk-by-chunk (\ie chunked prefilling), which reduces throughput due to lower GPU kernel efficiency, or by sharding the request state via parallelization, which also reduces throughput due to extra communication and synchronization overhead.
    % % of GPU computation due to sc the GPU computation idle extra communication cost and may also reduces the throughput especially when GPUs are not directly connected via high-speed connection hardware like NVLink.
    \item \textit{JCT-agnostic scheduling}: 
    Before prefill-only workloads, it was impossible to pre-determine the job completion time (JCT) of an LLM request, since the output length could be arbitrary depending on the random sampling. 
    In the lack of precise JCT knowledge, current LLM inference systems always use simple, JCT-agnostic, scheduling logic, such as first-come-first-served with some dynamic batching. 
    % Existing LLM engines use scheduling algorithms that are agnostic to job completion time (JCT).
    % This is reasonable for traditional generative requests, as the JCT depends on output length, which can be non-deterministic due to random sampling.
    However, for prefill-only workload, the output length is always 1 and thus the JCT can be accurately predicted under perfect knowledge, potentially allowing one to use JCT-aware scheduling to reduce the latency compared to JCT-agnostic scheduling.
\end{packeditemize}



% We refer to such workloads as {\em prefill-only}.
Thus, our goal is to build an LLM inference engine that specifically improves the performance (in latency and throughput) for prefill-only workloads in online serving scenarios.


A naive solution to address limitations introduced by two design choices of traditional LLM engines is to build a JCT profile offline based on the request length, and then in online phase, the LLM engine leverages this JCT profile to obtain the JCT of each incoming request, then schedule the waiting requests using JCT-aware algorithms (\eg shortest remaining job first) and discard the request state during the inference of that request.
This is a widely adopted solution in traditional deep learning systems~\cite{??,??}. 
However, this solution is not ideal in LLM scenario due to two limitations:
\begin{packeditemize}
    \item 
    Simply discarding the request state only allows the LLM engine to handle marginally longer requests without throughput reduction, as LLM inference itself has large GPU memory footprint.
    \item 
    Existing LLM engines use prefix caching, which leverage the cached state of one request to accelerate future requests that share the same prefix.
    Fully discarding the request state prevents such optimization.
\end{packeditemize}

% This makes the JCT  difficult to estimate a priori (as the request may hit the prefix cache).

To overcome these limitations, we propose \name, the first LLM inference engine tailored for prefill-only workload.

First, we propose \textit{hybrid prefilling} that allows \name to handle upto 7$\times$ longer requests without latency inflation.
Concretely, \name processes non-attention layers chunk-by-chunk but processes attention layers normally.
This is because most GPU memory usage in LLM inference comes from non-attention layers, and chunking them can significantly reduces the memory footprint, as these layers are all linear layers so each chunk can be computed independently with each other.
We note that, though hybrid prefilling benefits both prefill-only workload and traditional generative workload, it provides unique benefit for \name as it allows a prefill-only request to finish within a single round of LLM inference, making it possible to discard the request state without inflating the latency of future rounds of LLM inference.


Second, to enable prefix caching, we propose \textit{suffix request state discarding}: \name stores the request state of as many prefix tokens as possible on the GPU and discards the request state of suffix tokens when GPU memory is insufficient. 
We note that, this technique aims to align \name’s caching behavior with traditional LLM engines when the request state can be fully stored in GPU. 
We leave the optimization of selecting the optimal number of prefix tokens to cache for future work.



% Second, to enable prefix caching, we propose \textit{suffix request state discarding}: for an incoming request, \name  stores its state of as many \textit{prefix} tokens as possible in GPU, and discards the KV caches of remaining suffix tokens when the GPU memory is insufficient to fully cache the request state in GPU.
% We note that, this optimization aims to enable prefix caching in a way that aligns the caching behavior of \name with traditional LLM engines on short requests.
% We leave the optimization of deciding the best amount of prefix tokens that need to be stored in GPU in future work.
% % that caching behavior of \name only diverges with the traditional LLM engine when 




The introduction of prefix caching brings two new challenges to the scheduling algorithm:
\begin{packeditemize}
    \item How to estimate the JCT given that the JCT now depends on the prefix cache of LLM engine, which is constantly changing over time?
    \item How to increase the prefix cache hit rate?
\end{packeditemize}
We introduce \textit{continuous JCT calibration}, a unified solution for both challenges that can be seamlessly integrated into any JCT-based scheduling algorithm.
The idea of continuous JCT calibration is simple: during each scheduling step, we calibrate the JCT of each waiting request based on the current prefix cache. 
This allows the scheduling algorithm to obtain up-to-date JCT, while also increase the prefix cache hit rate, by timely prioritize those requests that can hit prefix cache and de-prioritize those requests that cannot.
% We note that, this scheduling algorithm may not necessarily achieve optimal prefix cache hit rate and we leave that to future work.
% To fully utilize prefix caching, the scheduling algorithm should be aware of the fact that the JCT changes over time (as the JCT depends on the prefix cache, which changes over time) and maximally increase the prefix cache hit rate.
% However, we found that traditional JCT-based scheduling algorithms achieve low cache hit rate in general, resulting in high latency and low throughput.
% This is because traditional JCT-based scheduling algorithms make decision based on the JCT when the request arrives, and thus fail to timely prioritize the requests when the LLM engine received prefix cache related to these requests, and deprioritize the requests when the corresponding prefix cache of these requests is evicted.

% The enabling of prefix caching challenges  to the online scheduling algorithm design: traditional JCT-based scheduling algorithms suffer from low throughput and high latency in prefix caching context since a significant portion of requests that could have hit prefix cache cannot hit the prefix cache 
% This is because JCT of one request is no longer a constant under the context of prefix cache: it decreases when a new request state that can be reused enters the prefix cache, and decreases when that request state is evicted.
% As a result, an ideal scheduling algorithm should timely prioritize those requests when their related prefix cache enters the LLM engine, and de-prioritize those requests when their related cache is evicted.

% This violates the assumption of traditional JCT-based scheduling algorithms that the JCT is roughly a constant.
% As a result, using a naive JCT-based scheduling algorithm leads to low throughput (due to low cache hit rate) and high latency (as the scheduler uses the JCT estimated during request arrival, which mismatches with the actual JCT when request being scheduled).


Further, to address the fairness and starvation issue in JCT-based scheduling algorithm, we also offset the JCT based on request waiting time, see \S\ref{??} for more details.
% We note that, continuous JCT calibration is a general component for JCT-based scheduling algorithms that makes them much more performant in prefix caching scenario.

% To address the low throughput and high request latency issue brought by traditional JCT-based scheduling, we propose \textit{continuous JCT calibration}, where \name re-estimates the JCT of all waiting requests based on current prefix cache condition.
% This technique, used together with traditional JCT-based scheduling algorithm like shortest remaining job first (SRJF), allows \name to improve the cache hit rate (as requests that hit prefix cache will have much lower JCT compared to other requests and thus will be prioritized by SRJF scheduler) and lower the request latency (as it guarantees that the SRJF scheduler always obtains the accurate JCT of the request being scheduled).
% Further, to address the starvation issue commonly appeared in SRJF-based scheduling, we offset the JCT by an aging term (more details in \S\ref{??}).

% We note that, this schedulithis technique does not achieve the optimal scheduling performance, and we leave that
% timely prioritizing those requests that can hit the prefix cache (as they tend to have much lower JCT compared to other requests) and supply JCT-aware scheduling algorithms like shortest remaining job first with accurate JCT estimation.

% As a result
% with the same prefix enters the prefix cache, and decreases when old request statwith the same prefix 
% it not feasible to predict the JCT of one request 
% creates new challenge to \name, as it makes the JCT of each request depends on what requests are executed previously breaks the assumption of traditional JCT-aware algorithms that the JCT of each request solely depends on the request itself and does not change with different request ordering.


% The enabling of prefix caching brings a new challenge to the scheduling algorithm.

% Due to prefix caching, the JCT of each request is now highly sensitive to request ordering.
% This is because the JCT of each request does not only depends on the request itself but also depends on the prefix cache available inside the inference engine.


% makes the JCT varies over time feasible to predict JCT a priori, as the prefix cache in LLM engines change over time as the state of new requests constantly evicts the state of old requests.
% % it decreases when new request states with shared prefixes are cached, and increases when caches are evicted).

% Facing this challenge, \name takes a pragmatic stance: where \name calibrates the JCT of all waiting requests based on the current prefix cache every time before scheduling.




We implement \name on top of vLLM, a state-of-the-art LLM inference engine. To ensure that generalizability of \name,  we implement hybrid prefilling via \texttt{torch.compile} so that \name can generalize to different LLM models, and implement suffix KV cache discarding without modifying hardware-related kernels so that \name generalizes to different hardware platforms.


We evaluate \name under 3 hardware platforms, 3 LLM models and 2 traces. Our evaluation shows that \name can handle 3$\times$ query-per-second  while still achieving lower average and P99 latency than the baselines.

To summarize, the contributions of this paper are:
\begin{packeditemize}
    \item  
    We identify a new trend in LLM use cases, where people use LLMs to substitute traditional deep-learning-based pipelines, and characterize a new workload -- \textit{the prefill-only workload} -- underlying these scenarios.
    \item We propose \name, the first LLM inference engine tailored for prefill-only workload, that  achieves 2$\times$ lower latency compared to baselines, and can handle upto $7\times$ longer requests without latency inflation.
\end{packeditemize}

% Hardware-wise, we focus on GPUs without hardware-accelerated inter-connections, as these GPUs are easier to maintain and more available in datacenter.
% \ion{This statement raises the question: are you actually focusing on these low end GPUs because your solution performs better on those GPUs? Keep in mind that Nvidia pushes people to use the high end GPUs for everything including inference. A better way to say it is that we provide significant performance improvements on all GPUs, and in particular on cheaper, reosurce constraint GPUs.} \lily{Another point, I guess workloads are generally running on low-end GPUs before LLM. So we just use the same GPU, replace the traditional model with LLM, that's why we run those models on low end GPUs. But agree with Ion, we should say it improves performance across all GPUs.}


%  and then observe the output probability distribution, \ie $P(\text{Output token is }\texttt{Yes})$ and $P(\text{Output token is }\texttt{No})$, where the sum of these two probabilities is 1.
% The recommendation application can then recommend the document with highest $P(\text{Output token is }\texttt{Yes})$.
% In other word, we observe two probabilities, where the  in other word, we only observe P(\texttt{Yes}) P(\texttt{No}).
% We then let LLM choose between ``Yes'' and ``No'' by letting LLM generate the output distribution on just two tokens, the ``Yes'' token and the ``No'' token in the vocabularity. 

% generate the distribution of the single output token,\textit{constraining} the selection of output token to only ``Yes'' and ``No'', and let LLM generate the output distribution of the 
% This allows people to the LLM to choose between options (\eg by )
%We identify a new workload behind such trend, in which \textit{LLMs only generate one single output token for each incoming request}.
% \ion{Most of the rest of this paragraph can be removed as it is repetitive. The one thing though to clarify is the "constraining the choice" part. Give an example.} This is because traditional applications are latency-sensitive, and generating just one single output token significantly reduces the latency of running one request, while still allowing LLMs to make decisions between multiple options (\S\ref{subsec:prefill-only-example}).
% Further, one can fully control the output behavior of LLM by simply constraining the choice of this single output token (while fully controlling the output behavior in traditional LLM workload remains challenging due to dependencies between output tokens).
% As a result, this approach builds a low-latency and robust foundation for people to build applications on top of LLMs.
% System-wise, the key characteristic of this workload is that it only requires running the prefilling stage of LLM inference.
% As a result, we name this workload \textit{prefill-only} workload. \lily{I feel it will be better to provide a concrete example here. For example, how is recommendation task formulated with LLM.}





% The first reason is that, existing LLM engines fully cache the request state in GPU, which significantly reduces the latency for traditional generative request but actually does not reduce the latency for short request and inflates the latency of long requests in prefill-only request.
% Concretely, for traditional generative request, fully caching the request state in GPU significantly reduces the delay of processing such request, because it requires multiple rounds of LLM inference (to generate multiple output tokens for this request) and caching the request state accelerates the LLM inference from the second round.
% However, for prefill-only request, fully caching the request state does not reduce the latency of this request, as it only requires one round of LLM inference. 
% Further, it may inflate the latency when handling long requests, because fully caching the request state limits the longest requests that the LLM engine can handle (since the request state is large), and thus, when handling a request longer than the limit, the LLM engines have to either process the input chunked-by-chunk, which inflates the request latency, or parallel the inference, which incurs extra communication cost and may inflate the request latency especially when GPUs are not directly connected
% via hardwares like NVLink.


% A natural optimization is thus to \textit{discard the request state}.
% This is a widely adopted solution in traditional deep learning system literature.
% However, this solution does not work well in LLM scenario due to two issues:
% \begin{packeditemize}
%     \item Future requests can reuse the request state to accelerate inference when they share the same prefix as the current request, and discarding the request state of current request prevents this acceleration.
%     \item Discarding the request state only allows the LLM to process marginally longer request ($1.6\times$ as shown in \S\ref{??}) without chunking the request or parallelizing the inference.
% \end{packeditemize}
% To address these two issues, we proposes two novel techniques:
% \begin{packeditemize}
%     \item \textit{Suffix request state discarding:} 
%     \name stores the request state of as many \textit{prefix} tokens as possible in GPU, and discards the KV caches of remaining suffix tokens.
%     This maximizes the chance of prefix cache hit and also allow \name to handle the long requests where their KV caches cannot be fully stored in GPU. 
%     \item \textit{Hybrid prefilling:} 
%     \name prefills non-attention layers chunk-by-chunk but prefills the attention layers normally.
%     This technique is enabled by a unique property in LLM: non-attention layers in LLM are all linear layers, which means that different chunks can be prefilled independently with each other in these layers.
%     This reduces the GPU footprint of non-attention layers, enabling the engine to handle upto $7\times$ longer requests without inflating their latencies.    
% \end{packeditemize}
% We note that hybrid prefilling is a general-purpose technique that elongates the maximum request length LLM engines can handle.
% However, this technique is a pre-requisite for suffix request state discarding, as it handles long requests \textit{within one round of LLM inference} and thus is necessary for suffix request state discarding (recall that request state discarding slows down LLM inference from the second round).

% The second reason for why existing LLM engines inflates the latency of prefill-only request is that existing LLM engines use scheduling algorithms that are agnostic to job completion time (\eg first-come-first-serve).
% The assumption behind is that the job completion time cannot be accurately predicted, which is true for traditional generative LLM requests, as the number of output tokens for each request is difficult to predict (or even non-deterministic due to randomness in sampling process).
% For prefill-only workload, however, this assumption no longer holds: the JCT of prefill-only request can be perfectly predicted (as the number of output tokens is always 1).

% As a result, a naive solution is to estimate the JCT when new requests arrive, and then use JCT-aware scheduling algorithms like shortest remaining job first (SRJF) to schedule these requests.
% However, such solution fail to timely prioritize the requests when they can hit the prefix cache, resulting in low prefix cache hit rate and thus high latency.
% This is because SRJF estimates the JCT only once, but the JCT of one request might change over time: it will become smaller if the current request introduces prefix caches related to this request, or become smaller if the current request evicts old prefix cache.


% To allow the sheduling algorithm to increase prefix cache hit rate, we propose \textit{continuous JCT calibration}, where we continuously calibrate the JCT of each request during each scheduling step, so that we can timely prioritize those requests that can hit prefix cache (as their JCT will become significantly lower) or deprioritize those requests that the caches they could have hit are evicted.
% Further, to address the starvation issue commonly appeared in JCT-based scheduling, we further offset the JCT by an aging term that guarantees the request will ultimately be scheduled.


% To incorporate the above optimizations, we propose \name.



% We argue that the latency of existing LLM engines manage are high when serving prefill-only workload.
% This is because existing LLM inference engines are designed for multiround LLM inference, where some of the design choices improve multiround LLM inference at the cost of inflating the latency of the first round (\ie prefilling) and thus increases the latency of prefill-only requests.
% Concretely, we characterize two design choices that inflates the latency of prefill-only requests:
% \begin{packeditemize}
%     \item \textit{Request state caching}: Existing LLM engines  fully cache the request state (in the format of KV caches or latent tensors) in GPU to accelerate the future round of LLM inference.
%     However, such caching does not reduce the latency of prefill-only requests as they only requires one round of LLM inference.
%     Further, the request state is large and fully caching it in GPU limits the longest requests the LLM engine can handle.
%     Thus, when there are long requests in the workload, the LLM engines have to process the input chunked-by-chunk, which inflates the prefill latency, or parallel the inference, which incurs extra communication cost and may inflate the request latency, especially when GPUs are not directly connected via hardwares like NVLink.
%     \item \textit{JCT-agnostic scheduling}: As the total rounds of LLM inference of one request depends on  number of output token, which is not fully predictable (and can even be non-deterministic) in traditional generative workload, existing LLM engine choose to use scheduling algorithms that are agnostic to job completion time (JCT), such as first-come-first-serve.
%     However, in prefill-only workload, it just require one round of LLM inference to handle one request, and thus the JCT can be perfectly estimated.
% \end{packeditemize}



% Thus, to reduce the latency of existing LLM engines on prefill-only workload, we propose two optimizations:
% \begin{packeditemize}
%     \item 
%     \textit{Discarding request state}:
%     As it only require one round of LLM inference to handle a prefill-only request, the request state does not need to be cached.
%     \item
%     \textit{JCT-aware scheduling}:
%     In prefill-only workload, there is only one round of LLM inference per request, which makes the JCT fully predictable, allowing us to reduce request latency leveraging JCT-aware scheduling algorithms such as shortest-remaining-job-first.
    
% \end{packeditemize}


% Though these optimizations are not new and are widely used in  traditional deep learning serving systems \ion{some references}, 
% we identify two practical challenges unique to the LLM workload:
% \begin{packeditemize}
%     \item Simply discarding the request state only allow the LLM engine to handle upto 1.6$\times$ longer requests, due to large intermediate tensors allocated by non-attention layers.
%     \item As LLM engines may store the request state past requests \ion{previous words are confusing} to accelerate future requests that share the same prefix (also known as prefix caching), the JCT of one request changes over time, as the KV caches of new requests can evict those of older requests.
%     \item Further, in the case when prefix caching is enabled, instead of fully discarding the request state for long requests, we should only partially discard the request state to maximize future reuse.
% \end{packeditemize}

% To address these challenges, we propose \name, the first LLM inference engine tailored for prefill-only workload.
% \name proposes three novel techniques to overcome the aforementioned challenges:
% \begin{packeditemize}
%     \item \textit{Hybrid prefilling:} \name prefills non-attention layers chunk-by-chunk but prefills the attention layers normally.
%     This reduces the GPU footprint of non-attention layers, enabling the engine to handle upto $7\times$ longer requests without inflating their latencies.
%     \item \textit{Suffix request state discarding:} For long requests, \name stores the request state of as many \textit{prefix} tokens as possible in GPU, and discards the KV caches of remaining suffix tokens.
%     This maximize the chance of prefix cache hit, while ensuring that caching behavior of \name only diverges with the traditional LLM engine when the request is too long for the KV caches to fully stored in GPU. 
%     \item \textit{Continuous JCT calibration:} \name continuously calibrates the JCT of each LLM request based on current LLM engine's prefix cache, so that the scheduling algorithm can make decisions using accurate JCT estimates.
% \end{packeditemize}





==> tex-files/misc.tex <==




\tightsection{Implementation}
\label{sec:implementation}
% \begin{packeditemize}
%     \item 5.1 Change detection workflow
%     \item Different from traditional change detection for RGB videos, change detection on satellite needs to handle cloud and illumination.
%     \item Introduce the workflow: cloud removal --> illumination alignment --> change detection --> encode the change
%     \item Cloud detection is known to be difficult and compute-intensitve due to the existence of thin clouds and faint haze.
%     \item The main insight of \name to reduce the computation cost is that it is tolerable for cloud detectors to wrongfully mark some cloudy areas as noncloudy and download them to the ground.
%     \item To reduce the compute cost, \name only trains cloud detector to detect those heavy clouds. This cloud can be easily detected by a cheap pixel-value-based decision tree algorithm, as there are designated bands that aim to monitor air quality and are sensitive to heavy clouds.
%     \item To further reduce the computation cost, \name detects cloud under low-resolution imagery.
%     \item \name will discard those images that are highly cloudy.
%     \item 5.3 Other modules in change detection
%     \item Linear regression for illumination alignment
%     \item Encoding and decoding the change --> layered image codec and jpeg header removal
%     \item Cloud detection on the ground --> Peder
% \end{packeditemize}

\begin{figure}[t!]
\centering
    \includegraphics[width=.9\columnwidth]{figures/dynamism.pdf}
    \vspace{-0.3cm}
    \tightcaption{Two satellite images captured consecutively do have similar content on the ground, but the pixel difference can still be significant due to cloud and illumination differences. Image © 2023 Planet Labs PBC.}
    \label{fig:satellite-imagery-dynamism}
\end{figure}




% \kt{Cloud detector on-board: no false positive (\ie wrongfully detect non-cloudy area as cloudy). Cloud detector: no false negative (cannot detect cloudy area as non-cloudy).}
% \kt{Two parts: the algorithm used in each module, and a SEPARATE paragraph on how to make them cheap enough to fit into storage}

% Different from detecting changes in image sequences captured by terrestrial sensors, change detection in satellite imagery needs to be robust to different cloud and illumination requirements. We briefly introduce the impact of cloud and illumination, and then explain how \name detect changes while being robust to different cloud and illumination conditions.
    



% \mypara{Cloud and illumination}
\mypara{Illumination and cloud}
% General-purpose change detection in image sequences has been widely studied, especially in video codec literature (\eg H.264~\cite{h264}) and video analytics literature (\eg~\cite{reducto,glimpse}).
% They yield great success in terrestrial cameras when two consecutive images in the image sequence are typically captured within several seconds or minutes. 
In satellite imagery, the time gap between two consecutively-captured images can be hours~\cite{planet} or days~\cite{sentinel-2}.
% This is because that the time gap between two consecutively-captured image for one geographical location is typically several days (\eg 1 day for Planet~\cite{planet} and 5 days in Sentinel-2~\cite{sentinel-2-revisit}).
As a result, two consecutive images in the image sequence can differ a lot in terms of pixel values due to different illumination condition and cloud condition (as illustrated in Figure~\ref{fig:satellite-imagery-dynamism}), making the general-purpose change detector (\eg~\cite{h264,h265,reducto,glimpse}) no longer suitable for satellite imagery compression.

Note that there are other potential sources (\textit{e.g.} sensor noise, image misalignment) that can also trigger large pixel differences. \name does not explicitly address them, as they only appear in raw data sensed by the satellite, which is not accessible in public datasets.

\mypara{Filtering out the cloud}
% \edit{This addresses shepherd's concern on why \name uses cheap cloud detector given that cloud detection is expensive}{
Previous work~\cite{kodan,satroi} observes that a wide range of applications (\eg autonomous road detection, precision agriculture) focus on the geographical content on the ground, allowing cloudy areas to be filtered out without impacting analytic results. 
Based on this observation, \name runs an on-board cloud detector to identify and filter out clouds.
However, as accurate cloud detector is too computationally expensive for on-board use (\S\ref{subsec:reference-compression}), \name runs a lightweight decision-tree-based cloud detector instead, which is a widely used cheap cloud detection algorithm that can still detect and filter out most clouds except for faint clouds and haze~\cite{pixel-cloud-detector-1,pixel-cloud-detector-2,pixel-cloud-detector-3}.
These faint cloud and haze are downloaded to the ground by \name (thus increasing the downlink usage of \name) but do not affect the analytic results of applications, as these applications will perform accurate cloud removal as an initial pre-processing step .
% }


% As a result, \name performs \textit{conservative cloud filtering} by only detect and filter out those easy-to-detect cloud. 
% This cheap cloud filter can filter out most of the clouds except for those faint cloud and haze.
% Those faint cloud and haze will be downloaded to the ground by \name.
% This decision is based on two insights:
% \begin{packeditemize}
%     \item 
%     That said, we acknowledge that it makes \name less applicable in cloud-sensitive applications.
% \end{packeditemize}





\mypara{On-board change detector}
Based on the aforementioned cloud filtering mechanism, \name then uses the following workflow to detect changes.
First, \name filters out cloud by detecting highly cloudy areas in the satellite imagery using a decision tree classifier, and remove this part of the data.
% (by filling the corresponding pixels with zero pixel value).
Second, \name drops those images if more than 50\% of the areas are filtered by the cloud filter.
% This is because a wide range of applications (\eg autonomous road detection, precision agriculture, etc.) treat highly cloudy data as of low value and will filter them out as they are focusing on the geographical content on the ground. Prior work also makes similar observations~\cite{kodan,satroi}. However, this does make \name less applicable in cloud-sensitive applications.
Third, \name aligns the illumination between the reference image and the captured image on less-cloudy areas using standard linear regression (since the illumination condition affects the pixel value linearly~\cite{illumination-model}).
At last, \name detects, encodes and downloads changes (details in \S\ref{subsec:reference-compression}).
% involves two phases: the ground contact phase and the image capturing phase.
% \begin{packeditemize}
% \item \textit{When contacting the ground}, the satellite downloads the changes for previously visited locations and updates the reference images for future locations (detailed reference image updating policy shown in \S\ref{??}).
% \item \textit{After capturing a image} for a geographical location, \name runs a cloud detector to remove clouds and aligns the illumination of captured image and the reference image. \name then detects changed areas and encodes the changed areas.
% % The satellite runs a cloud detection model that assigns cloud probabilities to pixels (details in \S\ref{subsec:cloud-detector}).
% % \item Aligning the illumination on the ground areas with the reference image.
% % \item Computing and encoding changes for non-cloudy regions. The data of cloudy areas will be discarded.
% \end{packeditemize}




\mypara{Encoding changed tiles}
\name encodes those changed tiles by selecting the changed tiles as region-of-interest and runs region-of-interest encoding on the whole image using an off-the-shelf JPEG-2000 encoder (Kakadu~\cite{kakadu}).
While encoding such images, \name makes sure that the bit spent on each encoded tile is a constant $\gamma$ by configuring the bit-per-pixel parameter of the Kakadu encoder as $\gamma$ times the percentage of tiles that are changed.
% region-of-interest encoding the region-of-interest, with the bit-per-pixel (bpp for short) as $\gamma$. The choice of $\gamma$ will be discussed soon.

\mypara{Choosing parameters for \name}
\name introduces two parameters: change detection threshold $\theta$ (\S\ref{subsec:reference-compression}) and bit-per-pixel $\gamma$.
\name chooses $\theta$ by profiling last year's data on one single location, and uses this parameter on this year's data for all locations.
\name then varies $\gamma$ to trade-off between downlink usage and imagery quality.




% \mypara{Fitting into on-board computation constraint}
% \name needs to detect cloud in order to remove cloudy areas and only download changes happened on the ground.
% However, accurate cloud detection is compute-intensive, as it typically requires using tens of layers of neural network~\cite{see-through-cloud}.
% \name instead leverages cheap decision-tree-based cloud detector, which can effectively detect thick cloud (since the temperature of heavy clouds significantly differs from the nearby ground and can be detected using the InfraRed band of satellite imagery), and runs fast on-board (faster than JPEG-2000 encoding).
% That said, this detector may fail to detect some light cloud (\eg haze).
% These areas will be detected as changed and downloaded to the ground, causing slight inflation on the downlink usage of \name.
%  \yh{Should we mention what's the impact on the download saving ratio after applying the faster cloud detection method? Maybe discuss this with junchen}



% \mypara{Cloud detector on the ground}
% \kt{Peder: can you fill in some detail on the cloud mask you generated in Sentinel-2 dataset?}



% This type of cloud can be detected from the InfraRed band of the satellites (which is commonly available in existing satellite constellations~\cite{planet,sentinel-2-bands}) using simple heuristics like the decision-tree algorithm.


% We note that those clouds that are not detected will instead be downloaded to the earth (as the cloudy area will have a much higher pixel value compared to its cloud-free pixel value in the corresponding reference image and will be detected as changed).
% that are commonly  by simple heuristics (\eg decision tree)





% We will illustrate why this workflow can stick with desired accuracy in \S\ref{??}.



% \subsection{Workflow}

% \begin{outline}
% \1 To detect change under varying cloud and illumination condition, \name use the following workflow on the satellite (Figure~\ref{fig:satellite-pipeline}).
%     \2 Cloud detection \& removal (assuming the cloud data can be discarded)
%     \2 Illumination alignment (we use a simple linear regression algorithm to determine the lighting change).
%     \jc{both alignment and cloud detection/removal come out of blue. downplay them if we don't touch the cloud/alignment-related stuff at all, to avoid confusion. if we touch them, please motivate the change in section 2 and 3 first.}
%     \kt{I motivated this challenge in section 3. I think it should not appear in section 2 as it is not a design question but rather an implementation question.}
%     \2 Change detection
%     \2 Encode and store the changes
% \end{outline}















% \subsection{Compute-efficient cloud detection}
% \label{subsec:cloud-detector}



% % \begin{table}[]
% % \footnotesize
% % \begin{tabular}{|l|l|l|l|}
% % \hline
% % & \begin{tabular}[c]{@{}l@{}}Computation\\ cost\end{tabular} & \begin{tabular}[c]{@{}l@{}}Correctly \\ classified pixels\end{tabular} & \begin{tabular}[c]{@{}l@{}}Accuracy\\ (IoU)\end{tabular} \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Inaccurate cloud detector\\ (decision-tree-based)\end{tabular} & 0.01 GFlops                                                & 96\%                                                                   & 0.5                                                                      \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Accurate cloud detector\\ (neural-network-based)\end{tabular}  & 1000 GFlops                                                & 99\%                                                                   & 0.9                                                                      \\ \hline
% % \end{tabular}
% % \caption{A cheap cloud detector can still correctly classify over 96\% of the geographical areas.}
% % \label{tab:inaccurate-cloud-detector}
% % \end{table}


% On the satellite, the most computationally intensive task within \name is cloud detection. Previous research~\cite{??} demonstrates that achieving accurate cloud detection involves neural networks with tens of layers, significantly exceeding the computational budget on the satellite.

% To address this challenge, \name observes that: 
% % First, by incorporating a cloud-free reference image as an auxiliary input, the cloud detector achieves comparable accuracy with much less computation. 
% % This is enabled by allowing the cloud detection algorithm to analyze pixel changes between the current image and the reference.
% % This approach is particularly effective in cloud detection, where clouds induce substantial pixel changes in comparison to the reference image.
% Second, while a compute-intensive cloud detector accurately handles complex scenarios (e.g., faint haze and cloud edges), these instances constitute only a small portion (around \fillme\%) of the observed satellite imagery.
% \kt{we need a measurement here}

% Building on these insights, \name employs a pixel-value-based decision tree to assign a cloud probability to each pixel. 
% Additionally, \name runs the decision tree on top of a downsampled image, as downsampling only makes the cloud filtering process of \name more conservative.
% This is because the highly cloudy pixels are very ``bright'' (\ie is of very large pixel value), while not-that-cloudy pixels are much darker. After downsampling, if these two types of pixels are downsampled together, they will result in a darker pixel, which will be labeled as not highly cloudy.


% To account for potential prediction errors from our cheap cloud detector, we make slight alterations to the illumination alignment~\ref{subsec:illumination-alignment} and change detection~\ref{subsec:change-detection} of \name, with the assumption that cloud detection errors commonly occur around a predicted cloudy probability of 0.5. 
% This property holds as our cloud detector uses decision tree algorithm, which generates a cloud probability near 0.5 when those pixels with similar pixel values in the training set are approximately half cloudy and half non-cloudy.



% On the satellite, the most computational expensive task of \name is the cloud detection.
% As prior work shows [??], it requires tens of layers of neural network to perform accurate cloud detection, which significantly exceeds the computation budget of the satellite.

% To handle this challenge, \name makes two observations.

% First, we observe that by the cloud detector can comparable accuracy while demanding significantly less computation power by introducing a cloud-free reference image as an auxiliary input.
% This is because the cloud creates a huge pixel change on the images, and the cloud detector can easily detect such pixel change using the reference image. 


% Second, though compute-demanding cloud detector can accurately detect cloud in intricate cases (\textit{e.g.} light haze and the boundary of the cloud), these cases only account for a small fraction (roughly 4\%) of the observed satellite imagery.




% Based on these observations, \name assigns a cloud probability to each pixel by running a pixel-value-based decision tree using the pixel value of both the reference image and the observed image.
% To further reduce the computation cost, \name runs the cloud detector on a image that are downsampled 4x on both width and height.



% \mypara{Illumination alignment}
% According to~\cite{illumination-model}, the illumination condition linearly alters the pixel value of the satellite imagery.
% % illumination on the pixel value is linear.
% In other word,
% Let $\mathbf{R}$ represents the reference image, $\mathbf{C}$ represents the current image. On cloud-free areas, we have $\mathbf{C}=k\mathbf{R}+d$, where $k$ and $d$ is two constants that do not change between different areas in the current image. 

% To obtain these two constants, \name runs standard linear regression on areas confidently identified as cloud-free (cloud probability less than a fixed constant $\alpha=0.3$).



% \subsection{Handling cloud detection errors}

% % We first categorize the error of cloud detector into two types:
% % \begin{packedenumerate}
% %     \item Boundary error
% %     \item Confusion error
% % \end{packedenumerate}



% First, as the illumination alignment and change detection relies on cloud detection results, we run these algorithms \textit{conservatively} so that potential cloud detection errors will be accounted as changes. 
% Concretely, during illumination alignment, . This approach ensures that cloudy pixels do not influence illumination alignment.









% \mypara{Change detection}
% \name detects changes by calculating the pixel difference between the observed image and the reference image in each block, and then marking those pixels with a difference greater than $\theta$ as changed.
% In our experiment, we fix $\theta=0.02$.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figures/staleness.pdf}
%     \caption{The amount of changes varies between different bands (B1 -- B12 in Sentinel-2 dataset).}
%     \label{fig:change-band}
% \end{figure}


\mypara{Handling different bands}
% \yhedit{Unlike traditional images that usually have 3 bands (R, G, and B), satellite images can have more than 10 bands~\cite{???}, including \fillme, \fillme, and \fillme. 
% In the Sentinel-2 dataset, each image has 12 different bands.
% }
Unlike traditional RGB images, satellite imagery typically has multiple bands and the amount of changes of different bands are different. 
% This figure is measured based on Sentinel-2 dataset on 1-year cloud-free areas in Washington State, where we define changed areas as those areas with pixel difference greater than 0.01, aligning with the definition in \S\ref{subsec:up-to-date-reference}.
% % \yh{Previouly you mentioned the difference threshold is 0.01, but here's 0.02}
% We perform linear regression on each band to highlight how fast the change increases with respect to each band.
For example, vegetation bands measure the concentration of chlorophyll (which is sensitive to temperature), while traditional RGB bands are less sensitive to temperature.
To handle such heterogeneity between bands, \name treats each band separately, which means that \name detects changes band-by-band and updates the reference images band-by-band, allowing \name to mark different areas as changed and download different amounts of changes for different bands.
% We empirically find that this optimization allows \name to further save 10\% downlink bandwidth, compared to download changes uniformly. \kt{The concrete number need to be measured again.}


\mypara{Handling bandwidth fluctuation}
% In the following discussion, we assume that the capacity of the downlink and uplink is predicted by a separate bandwidth predictor, and the goal of \name is to stick with the specified downlink/uplink capacity.
To handle uplink fluctuation, as \name locally caches the reference images, \name can randomly skip the updating of some reference images, and instead rely on the cached old reference images (at the cost of downloading more areas).
To handle downlink fluctuation, \name leverages the \textit{layered codec} feature, which allows \name to download less layers when downlink is limited (at the cost of degraded the image quality). 
The feature of layered codec is widely supported by existing imagery encoders on the satellite (\eg JPEG-2000 encoders~\cite{openjpeg,kakadu}).
% We note that \name downloads the same amount of layers for all locations that \name will download during one ground contact.
    
    % Concretely, while downloading the imagery, \name initially downloads the first layer for each location before proceeding to download the second layer for all locations, continuing in this manner until the contact with the ground finishes.
    % % and the next layer allows the ground to upload a parameter $b$, characterizing how many layers the ground is going to download for each location that the satellite captured according to the current downlink capacity, the satellite then sends $b$ layers of each location to the ground. 
    % This approach essentially downloads a similar amount of bits across different locations that will be downloaded during this ground contact. Acknowledging that downloading different amount of bits for different locations can be better, \name leaves this improvement to future work.


% \mypara{}


% \mypara{Handling downlink alteration}
% \name relies on the \textit{layered codec} to handle the alteration of downlink.
% The characteristic of layered codec is that: by encoding the images to multiple layers, \name can trade-off between downlink bandwidth and the quality of downloaded imagery quality gracefully: the ground can download more layers to receive high-quality imagery imagery when having sufficient downlink bandwidth, or download less layers to the ground when the downlink bandwidth is limited.
% The feature of layered codec is widely supported by existing imagery encoders on the satellite (\eg JPEG-2000 encoders~\cite{openjpeg,kakadu}).

% Concretely, while downloading the imagery, the satellite allows the ground to upload a parameter $b$, characterizing how many layers the ground is going to download for each location that the satellite captured according to the current downlink capacity, the satellite then sends $b$ layers of each location to the ground. 

% We note that this parameter $b$ is the same across different locations that will be downloaded during this ground contact. Acknowledging that downloading different number of layers for different locations may be more optimal, \name leaves this improvement to future work.



% Technically, we leverage the layered codec feature of Kakadu~\cite{kakadu} (a JPEG-2000 encoder) and specify

% To handle downlink alteration, \name encodes the imagery using \textit{layered codec}, allowing the ground to gradually improve the quality of the received imagery when downloading more bits to the ground.

% imageencodes the images into different layers, and the ground can specify how many layers it wants to download during ground contact time.
% download more layers if the bandwidth
% let the ground specify that how many bits need to be downloaded for each location 
% and the ground can download \textit{arbitrary bits} from any location.

% We calculate the changes in each 16x16 block as the current satellite encoding algorithm (\textit{i.e.} JPEG-2000) encodes the images block-by-block and the minimum size of each block is 16x16.





% As our cheap cloud detector may generate the wrong prediction, we handle this prediction error using the following policy:
% \begin{packeditemize}
%     \item When aligning illumination, \name operates on areas that are certainly non-cloudy (cloud probability smaller than a constant $\alpha=0.2$).
%     This allows \name to align the illumination on the ground without being affected by cloudy pixels.
%     \item When detecting changes, \name only eliminates those areas that are certainly cloudy, defined as those areas with cloud probability greater than $1-\alpha$.
% \end{packeditemize}

% Note that the policy above assumes that the cloud detection makes error when the predicted cloudy probability is close to 0.5.
% This is true for our cloud detector as our cloud detector leverages decision tree algorithm, which generates the predicted probability by directly counting the number of cloudy observations (under the current decision) and the number of non-cloudy observations.


% Selective Accuracy: The examination of cloud occurrences highlights that intricate cases, such as those involving light haze and water reflection, account for a mere fraction of the satellite's coverage (roughly 4\%). Conversely, a less sophisticated cloud detector achieves accurate cloud detection in over 96\% of the observed area. Thus, the high-cost cloud detector's advantages are mainly relevant to a minimal subset of circumstances.


% Informed Detection: Leveraging a cost-effective cloud detector as its backbone, \name capitalizes on the reference image to augment detection capabilities. By judiciously combining these resources, we strike a balance between accuracy and computational efficiency.

% \subsection{Encoding the changes}

% \name encodes the changed areas with a fixed bit-per-pixel $b$ by leveraging the region-of-interest encoding feature of an JPEG-2000 encoder (Kakadu~\cite{kakadu}).

% detected changes with a fixed encoding quality.
% This fixed quality is decided by a parameter $b$, where $b$ describes the file size divided by the number of pixels of changed areas (\ie bit-per-pixel on changed areas).

% As a result, \name uses the region-of-interest encoding feature of  while constraining the encoded file size to be $b$ times the number of changed pixels.

% The region-of-interest encoding of Kakadu accepts a parameter $b'$ that describes the file size divided by the amount of pixels of all areas.
% As a result, we let $b' = b \times \frac{\text{\# of changed pixels}}{\text{\# of all pixels}}$ 

% \subsection{Decoding the image}

% \name only downloads the changed areas.
% For the areas that are not labeled as change, \name will reconstruct those areas by using 
% \begin{equation*}
%     k\mathbf{R}+d,
% \end{equation*}
% where $\mathbf{R}$ is the reference image and $k, d$ is the illumination coefficients in \S\ref{subsec:illumination-alignment}.

% Note that while the change detection process uses the onboard version reference image $\mathbf{R}$, which is a low-resolution image (\S\ref{subsec:reference-compression}), we use the original version of the reference image $\mathbf{R}$ on the ground to reconstruct the unchanged areas.




% \section{Safeguarding mechanism in \name}

% \subsection{Handling cloud prediction error}

% \name leverages a cheap decision-tree-based algorithm to detect clouds so this cloud detector will generate errors.
% We note that these errors are mainly cloudy pixels that are wrongfully labeled as non-cloudy (since \name detects cloud conservatively) and these pixels will be labeled as change and downloaded to the ground.

% As a result, the wrong prediction of cloud detectors will be safely downloaded to the ground.

% \subsection{Handling change detection error}

% Since \name leverages a low-resolution reference image to detect changes, \name may miss some changes that happen on the ground.
% As a result, there will be some areas in the satellite imagery that are changed but are not downloaded.



% \mypara{Guaranteed downloading}
% As some changed tiles will not be downloaded to the ground by \name (\S\ref{subsec:reference-compression}), \name guarantees the downloading of cloud-free imagery in its entirety at a low frequency (once every month).



\mypara{Updating reference images}
\name needs to constantly update its reference images.
A naive design is to constantly patch the reference image with newly observed changes, similar to how a video encoder updates its reference images~\cite{h264,h265}.
However, we found that this approach will gradually degrade reference image quality, since each patch will introduce some artifact to the reference image (which is caused by \name's imperfect illumination alignment due to low reference image resolution) and such artifact accumulates.

% \edit{Rename the reference image updating technique to whole image downloading, to avoid the confusion that the downloading technique provides monthly downloading guarantee}{
As a result, \name instead acquires reference images by \textit{whole image downloading}: for each location, \name downloads the first cloud-free image observed by any satellite in the constellation. 
After this, \name will stop whole image downloading for this location for a month.
% As a result, \name instead obtains the reference images by \textit{guaranteed downloading}: for each location, \name will guarantee the downloading of the first cloud-free image observed by any of the satellites in the constellation in its entirety, and then turn off the guaranteed downloading for this location for one month.
This operation will not introduce large overhead in large-scale LEO constellations, as the overhead of guaranteed downloading is fixed (at most 12 times a year) and will be evenly spread out by all satellites in the constellation.


% \edit{This clarifies that the frequency of whole image downloading can be much lower than once per month}{
% Note that though \name starts to download a new reference image after the latest image is one-month old, the frequency of whole image downloading is strictly less than once per month (as only cloud-free image can be reference) and can be much lower for small-scale constellations in practice.
% For example, if the constellation only contains one satellite, the frequency of whole image downloading is once per 80 days in average, roughly 4 times a year, where the 80 days estimation comes from the fact that \name tries to download a new reference for a location after 30 days, and the satellite needs to wait for an extra 50 days in average (\S\ref{subsec:up-to-date-reference}) for a new cloud-free reference.
Note that although \name starts to find a new cloud-free image as reference one month after observing the last reference image, the extra time it takes to actually find such cloud-free image can be excessively long, which indicates that the actual downloading frequency can be much lower than once per month.
In the extreme case, assuming that the constellation contains only \textit{one} satellite, the frequency of whole image downloading will be once every 81 days in average --- only around 4 times a year, where this 80-day estimate comes from the fact that \name starts updating the reference after one-month wait, together with an additional wait time of 51 days in average (\S\ref{subsec:up-to-date-reference}) to actually observe such cloud-free reference image.
% }
% This is because Earth+ will wait for at least one month before starting to download a new reference, and the extra time required after one month of waiting to find a new reference can be excessively long for the small-scale constellation, as even in the average case it takes 50 days for a single satellite to observe a new cloud-free reference (shown in Sec. 3)

% A side benefit of guaranteed downloading is that it guarantees any part of the Earth will be eventually downloaded.



% Concretely, for a given location, after downloading only changed tiles for a month, \name will let the satellite download the next cloud-free image captured by any satellite at this location in its entirety.
% This mechanism guarantees that even if there are some changes that \name fails to detect, \name can still download these changes by downloading the images in their entirety.

% \mypara{Guaranteed downloading}To handle this issue, \name performs guaranteed downloading, where \name periodically downloads a cloud-free image \textbf{\textit{in its entirety}} once every $t$ days, with a bit-per-pixel of $b'$.
% This guarantees that any area in 
% We note that the first reference image of \name is also obtained with this mechanism.





% \kt{Goal: nuggets, reference image quality, resolution v.s. change detection threshold change-by region; if a change is missed, safe-guarding mechanism to save this missed change?}
% \kt{Uplink quality is too low --> can satellite realize that the quality is too low? Random fix?}

% \kt{Why uplink is small? Reason 1: every location --> lowest resolution: rightly fit the predicted spatial granularity of change}
% \kt{If the prediction is wrong, we have someway to detect it: periodically better resolution and see if the detection is better}
% \kt{End-to-end evaluation}
% \kt{Measurement: a very }





% \subsection{Safeguarding potential errors}

% \begin{outline}
% \1 The cheap cloud detector of \name may still generate errors.
% \1 We categorize 
% \1 To safeguard against such errors, we provide two mechanisms.
% \1 Safeguard mechanism 1: when in doubt if an area is cloudy / changed, just download that area.
%     \2 Concretely, \name will have 
% \1 Safeguard mechanism 2: when an area is not downloaded for e.g. 2 months, download it regardless of its cloud condition.
% \end{outline}


% \begin{packeditemize}
% \item Cloud removal
% \item Need to mention the assumption that cloudy data are not useful (this need to be justified much earlier)
% \item Illumination alignment
% \item Change detection
% \item Encoding
% \end{packeditemize}


% \subsection{Incoporating resource constraint on the satellite}

% \begin{packeditemize}
% \item Save compute: decision-tree-based cloud detector on the downsampled satellite image.
% \item Save storage: downsampled version of the reference image.
% \item Errors WILL occur. Error handling policy: when in doubt, just download.
% \end{packeditemize}


% \subsection{Handling subtle but consistent change}

% \begin{packeditemize}
%     \item Guarantee that each area WILL be downloaded once every X months.
% \end{packeditemize}






% \section{Safeguarding mechanisms}

% \subsection{Conservative cloud detection}


% \subsection{Full image downloading}
